EBBINNOT: A Hardware Efficient Hybrid Event-Frame Tracker for Stationary Dynamic Vision Sensors

As an alternative sensing paradigm, dynamic vision sensors (DVS) have been recently explored to tackle scenarios where conventional sensors result in high data rate and processing time. This paper presents a hybrid event-frame approach for detecting and tracking objects recorded by a stationary neuromorphic sensor, thereby exploiting the sparse DVS output in a low-power setting for traffic monitoring. Specifically, we propose a hardware efficient processing pipeline that optimizes memory and computational needs that enable long-term battery powered usage for IoT applications. To exploit the background removal property of a static DVS, we propose an event-based binary image creation that signals presence or absence of events in a frame duration. This reduces memory requirement and enables usage of simple algorithms like median filtering and connected component labeling for denoise and region proposal respectively. To overcome the fragmentation issue, a YOLO inspired neural network based detector and classifier to merge fragmented region proposals has been proposed. Finally, a new overlap based tracker was implemented, exploiting overlap between detections and tracks is proposed with heuristics to overcome occlusion. The proposed pipeline is evaluated with more than 5 hours of traffic recording spanning three different locations on two different neuromorphic sensors (DVS and CeleX) and demonstrate similar performance. Compared to existing event-based feature trackers, our method provides similar accuracy while needing approx 6 times less computes. To the best of our knowledge, this is the first time a stationary DVS based traffic monitoring solution is extensively compared to simultaneously recorded RGB frame-based methods while showing tremendous promise by outperforming state-of-the-art deep learning solutions.

==> 02_B_KF.tex <==
\subsubsection{Kalman Filter based Tracking}
A classical application of Kalman Filter (KF) in computer vision involves estimating the position of a detected object in a two-step process - prediction of object position and correction to refine the estimates considering noise measurements~\cite{Camunas8088365}. Object tracking using KF (KF Tracker) as implemented in~\cite{LinLin2015}, associates detections to the track of the same object by estimating the track’s location in each frame, and determining the likelihood of assignment of tracks and detections using Hungarian Assignment. Unassigned detections seed a new track and a count of visibility of all tracks is maintained to delete tracks which may have left the scene, when it remains invisible beyond a certain number of frames. Estimating the number of computations performed per frame and the memory required to track objects is an important step to assess the suitability of a tracker for power and area constrained applications such as remote surveillance. Since our proposed OT method in Section \ref{sec:materials} is closely related to KF, we detail the derivation of the number of computations per frame, $C_{KF}$ (based on \cite{Valade2017ASA,Munkres1957AlgorithmsFT}), for KF Tracker as follows:

\begin{align}
\label{eq:KF}
&C_{KF} =  N_T ( C_{p} + P_{a}C_{c} +P_{uat}C_{u} + C_{cost}) \notag\\ &\indent\indent\indent+ N_{obj} ( P_{ua}C_{new}) +  C_{ha} \notag\\
&C_{p}	= 4m^3 + 3m^2 + 2mn  \notag\\
&C_{c}	= 6m^3 + 6m^{2}n + 2mn^2 + 3m^2 + 7mn + m + n  \notag\\
&C_{u} 	= 2, C_{new}= 1\notag\\
&C_{cost}   	= 4n^3 + 2m^{2}n + 2mn^2 + 5n^2 + 5  \notag\\
&C_{ha}= 1/6 (11N_{obj}^3 + 12N_{obj}^2 + 31N_{obj})
\end{align}
where $N_T$ and $N_{obj}$ are the average number of tracks and objects per frame respectively, $P_a$	is the probability of assignment of detection to track, $P_{ua}$ and $P_{uat}$ are the probabilities of unassigned detection and track respectively, and $m$, $n$ are the sizes of state  and measurement vectors respectively. $C_{p}$, $C_{c}$, $C_{u}$, $C_{ha}$, $C_{cost}$, $C_{new}$ in eq.~\ref{eq:KF} represent the average number of computations per frame involved in the logic for prediction, correction, track update, Hungarian assignment, cost estimation of assignment of detection/track and seeding a new track respectively. Likewise, based on \cite{PageKF}, we define the memory requirements for KF per frame, $M_{KF}$, as follows:
\begin{align}
\label{eq:KF_m}
&M_{KF} =  N_T \times WS(5m^{2} +m(3n + 1) + n^{2} + 2n) \notag\\ &\indent\indent\indent+ ( A \times B)
\end{align}
where, $A\times B$ is the dimension of a binary frame and $WS$ is the word size. Then, assuming $A=240$, $B=180$, $WS=32$ and $N_T=8$, the estimated storage needed would be approximately $6.8$KB.

==> 02_background.tex <==
\section{Background}
\label{sec:background}
\subsection{Neuromorphic Vision Sensor (NVS)}
A NVS or event camera, unlike a traditional image sensor with fixed frame rate, operates by detecting temporal contrast (or change in log-intensity) at all pixels in parallel. If the change is larger than a threshold, it generates an asynchronous digital pulse or spike or event with a timestamp and a pixel location associated to it. Further, a polarity is assigned to each and every event according to the direction (increase or decrease) of contrast variation. This type of signalling is referred to as address event representation (AER). These changes in the format of data produced hence require a paradigm shift in the algorithms required for processing the input for various applications, opening up a whole new avenue in engineering\cite{nvs-review,DBLP:journals/corr/abs-1904-08405}.

Mathematically, an event can be modeled as $[e_i = (x_i, y_i, t_i, p_i)]$ where $(x_i,y_i)$ represents the event location or address on the sensor array, $t_i$ represents the timestamp of the event and $p_i$ represents the polarity associated to it~\cite{brandli2014live}. The associated timestamps to each event have microsecond resolution with quick readout rates ranging from $2$ MHz to $1200$ MHz. The event camera has an in-built invariance to illumination, since it detects temporal contrast change  largely cancelling out the effect of scene illumination. In short, the variation in log intensity represents the variation in reflectance due to the movement of the objects in the view. 

\subsection{Tracking}
\label{sec:tracking}
Visual tracking is a fundamental operation in video processing\cite{tracking-review}, and is critically needed in applications ranging from autonomous vehicles to traffic surveillance. For event driven NVS, one can perform tracking either directly on events or generate frames (at fixed time interval or at fixed event counts\cite{jyoti-frontiers}) to apply conventional frame driven techniques. We next review classical examples of three such algorithms.

\input{02_B_KF}


\subsubsection{Event based Tracking}
\textbf{(1) Event based Mean Shift (EBMS) tracking} - is a representative algorithm that operates directly on events with a good computational performance. The mean shift tracking approach used on frames in early 2000s~\cite{comaniciu2000mean} was modified for application on event clusters in~\cite{delbruck2013robotic}. These event clusters represent the moving objects with each having events occurring in close proximities. The new cluster positions and velocities are modeled with the help of mixed equation of old positions and velocities and the new incoming event location. The cluster is considered active only if it contains a threshold number of events, and is lost if no new events are found inside it for a threshold period. This method is advantageous since the events occur only at few pixels and the majority of the scene is unchanged. 

The total number of computes per frame ($C_{EBMS}$) and the memory requirement in bits ($M_{EBMS}$) for the EBMS \cite{AuthorsEBBIOT} algorithm are given by,
\begin{align}
\label{eq:EBMS}
    C_{EBMS} =& \overline{N}\times [9~\overline{CL}^2+{(169+16~\gamma_{merge})}~\overline{CL} +11]\notag\\
    M_{EBMS} =& 408 CL_{max}+ 56
\end{align}
respectively, where $\overline{N}$ is the average number of events per frame, $\overline{CL}$ is the average number of active clusters at any given time ($\approx \overline{N_T}$), $\gamma_{merge}$ is the probability of two clusters merging, and $CL_{max}$ is the maximum number of potential clusters.

\textbf{(2) Event based Feature Tracking (EvFT)} is required by several machine-vision tasks such as object segmentation, visual odometry, scene understanding, optical flow estimation rely heavily on feature detection and tracking on the image plane. While a key feature of event camera is its intrinsic immunity to motion blur, a feature tracker in \cite{Kostas-flow} uses motion blur induced by projection of events onto a 2D plane to extract event information and flow estimation. Data association between events is estimated by using a Gaussian model for probabilistic association, based on the assumption that events from the same image point are clustered together for a given correct deblurring. 
\cite{Kostas-flow} implements an event-based feature tracker based on probabilistic associations between features and events. A variable time windowing scheme is used to group events and to create trackers out of the detected features, using lifetime determined using the length of the optical flow. The primary outputs from the tracker are the positions and optical flows of the tracked features. Persistence of tracks is increased by computing the affine transformation for each feature with respect to the starting time. An expectation-maximization (EM) scheme is used to compute probabilities (weights) for data association for a given optical flow, followed by determining the expectation over these probabilities to compute the optical flow. In section \ref{subsec:rpn_comparisons}, we describe how we utilize this event-based feature tracker for region proposal in our proposed flow and compare it with our proposed region proposal method, with respect to accuracy and computational complexity, whereby we show the impracticality in implementation of feature tracker for the targeted low power high efficiency IoT application.
%The authors in~\cite{AuthorsEBBIOT} derived a formula for the number of computes per frame ($C_{EBMS}$) and memory requirement in bits ($M_{EBMS}$) for the EBMS algorithm.
%\begin{align}
%\label{eq:EBMS}
%    C_{EBMS} =& \overline{N}\times [9~\overline{CL}^2+{(169+16~\gamma_{merge})}~\overline{CL} +11]\notag\\
%    M_{EBMS} =& 408 CL_{max}+ 56
%\end{align}
%where $\overline{N}$ is the average number of events per frame, $\overline{CL}$ is the average number of active clusters at any given time ($\approx \overline{N_T}$), $\gamma_{merge}$ is the probability of two clusters merging and $CL_{max}$ is the maximum number of potential clusters. Assuming the past 10 positions of cluster are used for the current velocity calculation, $CL_{max}=8$ and for our dataset, $\overline{CL}\approx 2$, $\gamma_{merge}\approx0.1$ and $\overline{N}\approx 650$, EBMS requires 252 kops per frame which is $\approx 500\times$ higher than EBBIOT~\cite{AuthorsEBBIOT}, and a memory of $3.32$ kB, which is nearly negligible.

% The total memory required for EBMS is $3.32$ kB which is again negligible compared to the earlier processing blocks for noise filtering.

\subsubsection{Deep learning based Tracking}
\label{subsec:SiamMask_Intro}
%The word Siamese was taken from Siamese twins, which refers to conjoined twins. Since, They hailed from Siam(Thailand), Therefore referred as siamese. Hence, Siamese was phrase for conjoined twins. 
Use of deep neural networks (DNN), specifically one-shot learning has demonstrated success in object tracking tasks. 
For standard RGB frames, Bromley \etal \cite{novel-siamese} demonstrated first success after using Siamese-inspired neural network architecture to verify signatures. In general, Siamese architecture resembles the physical structure of conjoined twins. Following the significant progress in DNNs, these architectures turned out to be efficient for image matching and verification using one-shot learning \cite{Koch2015SiameseNN}. With the development of deep convolutional neural networks (CNNs) and availability of large data sets for training, fully convolutional Siamese (SiamFC and SiamRPN) networks \cite{DBLP:FC-SiameseNetworks} turned out to be efficient online tracking architectures using similarity matching.
\par
Apart from establishing itself as one of the state-of-the-art on the popular visual object tracking (VOT 2018) benchmark, SiamMask \cite{DBLP:Siammask} is popular for its simplicity, speed and online learning. Unlike traditional CNNs, it solely relies on initial bounding box coordinates of the target in the first frame of the video stream, which is referred to as an \emph{exemplar image}, and estimates object position to generate segmentation mask in subsequent images. SiamMask works on the principle of similarity matching between an exemplar image and a search image. To initialize this tracking process for the $n^{th}$ frame, we provide ground truth information for the object-of-interest, i.e. exemplar image, and the subsequent $(n+1)^{th}$ frame is treated as the search image. % can be written as "the subsequent $(n+1)^{th}$ frame is treated as the search image" ? 
\par
Based on the above input, SiamMask generates an object mask and its corresponding anchor box by max-min techniques \cite{DBLP:Siammask} on the search image, as shown in Figure \ref{fig:SiamMask_Mask_AnchorBox}. This current anchor box information along with the $(n+1)^{th}$ frame is used as the exemplar image to track the object-of-interest in the $(n+2)^{th}$ frame. This process continues and objects are tracked for the rest of the sequence. However, SiamMask fails to track in case of missing object-of-interest \cite{DBLP:Siammask}. To avoid such scenarios, only search images with object-of-interest are made to be part of the test sequence, and thus provide the best-case scenario for SiamMask in our evaluation.
%Thus, we  eliminate the false positives and provide the best case scenario for SiamMask in our evaluation.
\par
 Belonging to the same family, SiamRPN++ \cite{SiamRPN++_Li_2019_CVPR} is a more recent tracking framework that outperforms SiamMask on the VOT2018 dataset. Thus, we also compare the proposed NVS object tracking pipeline with both these Siamese DNNs, applied to simultaneously recorded RGB frames for a close comparison. 

\begin{figure}[t]
\centering     %%% not \center
\includegraphics[width=9cm]{img/SiamMask_RGB_FOV90_Mask_anchorbox.jpg}
 \caption{SiamMask tracking a vehicle, mask generated is denoted by red colour and corresponding anchor box calculated using max-min method in green colour}
\label{fig:SiamMask_Mask_AnchorBox}
\end{figure}


%Practically, Exemplar image is the object in previous frame which needs to tracked in the search image.


%However, SiamMask is bound to fail in case of motion blur and no-object instances in future frames \cite{DBLP:Siammask}, as will be shown later for standard RGB cameras. 
%On the other hand, these problems are naturally absent in the event stream and we propose applying SiamMask after fixed interval time sampling.  

%Siamese networks were initially developed for image matching such as Signature verification in early 90s 
%Siamese architecture demonstrated their ability to perform similarity matching at various levels which include signature Matching , face recognition as like a bouncer in club compares face in ID to Face of a person, and comparing two image patches . 
%Siamese architecture was successful in achieving human level performance in activities such as Recognition and 

==> 04_Results.tex <==
\section{Results}
\label{sec:results}
In this paper, we wanted to compare performance of NVS with a standard RGB camera; however, such a dataset is not available as far as we know. Consequently, it demanded the acquisition of event-based data and RGB data from a real traffic scenario for training, validation and  testing \footnote{Dataset: \url{https://zenodo.org/record/3839231}}. Further, in order to test the system performance, we employed two evaluation metrics for object detection and classification.

\begin{itemize}
    \item \textbf{F1 score for detection performance:} We have already discussed in Section~\ref{sec:NNDCrp} that $IoU$ is an effective metric for evaluating the detection accuracy. The tracker annotation can be matched with GT annotation to get $IoU$ in order to conclude whether it represents a true object BB ($IoU>IoU_{th}$) or a false object BB according to the threshold ($IoU_{th}$). Thereafter, we sweep $IoU_{th}$ from $0.1-0.9$ in steps of $0.1$ to find out precision and recall averaged over the entire duration of the recording. We further calculate F1 score for each recording as follows:
    \begin{align}
\label{eq:f1_score}
    &F1_{iou}^j=2\frac{P_{iou}^j\times R_{iou}^j}{P_{iou}^j+ R_{iou}^j}\notag\\
    &F1_{iou}^{wtd} = \frac{\sum_{j=1}^{K}N_{tracks}^j\times F1_{iou}^j}{\sum_{j=1}^{K}N_{tracks}^j}
\end{align}
    Here, $P_{iou}^j$ and $R_{iou}^j$ are precision and recall for the recording $j$ at $IoU=iou$, $N_{tracks}^j$ represents number of tracks in recording $j$ and $F1_{iou}^{wtd}$ represents the weighted F1 score for all the $K$ recordings, $j=1,\dots, K$. Thus, we examine the detection performance of our dataset in terms of $F1^{wtd}$ swept over $IoU$.
    \item \textbf{Overall accuracies for classification performance:} We calculated both the per-sample and per-track classification accuracies. In order to calculate the predicted class of a track, we recorded the statistical mode of the classification output for all the samples in the respective track. Further, we defined two types of accuracies: overall balanced and overall unbalanced. The former represents the average of class-wise accuracies to have a definitive evaluation measure while dealing with the dataset imbalance. The latter represents the widely used average accuracy for all the samples in the dataset regardless of class distribution. 
\end{itemize}

 The rest of this section presents the data collection process and preparation for training our classification model, followed by  the evaluation of the proposed noise filtering technique. Then, we evaluate the three different RP networks and provide insights about the hybrid RP network for the pipeline. Next, we compare the OT and KF trackers, followed by comparing the full EBBINNOT pipeline with event-based and frame-based state-of-the-art methods in section \ref{sec:statecompare}. Finally, we compare the computations and memory usage of proposed EBBINNOT with other methods.
\subsection{Experiments with DAVIS}
\label{subsec:Experiments-on-DAVIS}

\begin{table}[t]
\caption{Mean object sizes at different recording sites}
\centering
\begin{tabular}{ccccc}
\hline
\textbf{Recording Site} & \textbf{Car/Van} & \textbf{Bus} & \textbf{Bike} & \textbf{Truck} \\ \hline
\textbf{Site 1} & $16\times42$ & $31\times94$ & $15\times21$ & $22\times50$ \\
\textbf{Site 2} & $25\times47$ & $52\times107$ & $17\times22$ & $35\times61$ \\
\textbf{Site 3} & $34\times82$ & $64\times180$ & $26\times44$ & $50\times104$ \\ \hline
\end{tabular}
\label{tab:class_sizes}
\end{table}

\begin{table*}[h]
\caption{DAVIS traffic dataset.}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccc}
\hline
{\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Recording \\ Site\end{tabular}}} & {\color[HTML]{000000} \textbf{Duration}} & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Time \\ of Day\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Lens \\ Resolution\end{tabular}} & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Number of \\ Events\end{tabular}}} & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}\# of Recordings\\ in Training $\mid$ Testing\end{tabular}}} & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Car/Van  \\ (Samples $\mid$ \\ Tracks)\end{tabular}}} & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Bus  \\ (Samples $\mid$ \\ Tracks)\end{tabular}}} & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Bike  \\ (Samples $\mid$ \\ Tracks)\end{tabular}}} & {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}Truck  \\ (Samples $\mid$ \\ Tracks)\end{tabular}}} \\ \hline
{\color[HTML]{000000} \textbf{Site 1}} & {\color[HTML]{000000} 2h11m} & {\color[HTML]{000000} 3PM, 4PM} & 12mm & {\color[HTML]{000000} 201M} & {\color[HTML]{000000} 6 $\mid$ 2} & {\color[HTML]{000000} 18232 $\mid$ 379} & {\color[HTML]{000000} 8081 $\mid$ 165} & {\color[HTML]{000000} 1378 $\mid$ 35} & {\color[HTML]{000000} 2256 $\mid$ 47} \\
{\color[HTML]{000000} \textbf{Site 2}} & {\color[HTML]{000000} 2h25m} & {\color[HTML]{000000} 3PM, 4PM} & 6mm & {\color[HTML]{000000} 132M} & {\color[HTML]{000000} 6 $\mid$ 3} & {\color[HTML]{000000} 16918 $\mid$ 382} & {\color[HTML]{000000} 8019 $\mid$ 177} & {\color[HTML]{000000} 1604 $\mid$ 39} & {\color[HTML]{000000} 2513 $\mid$ 56} \\
{\color[HTML]{000000} \textbf{Site 3}} & {\color[HTML]{000000} 1h} & {\color[HTML]{000000} 3PM} & 8mm & {\color[HTML]{000000} 50M} & {\color[HTML]{000000} 2 $\mid$ 1} & {\color[HTML]{000000} 6514 $\mid$ 209} & {\color[HTML]{000000} 1201 $\mid$ 27} & {\color[HTML]{000000} 512 $\mid$ 22} & {\color[HTML]{000000} 501 $\mid$ 15} \\ \hline
\end{tabular}%
}
\label{tab:dataset_statistics_overview}
\end{table*}

The desired location for the traffic recordings was a high, perpendicular view from the road near intersections. In this regard, three places shown in Figure~\ref{fig:Locations}, were chosen for data collection using DAVIS. Further, we also captured RGB recordings for simultaneous comparison with the purely frame-based tracking SiamMask, as shown in Figure \ref{fig:Dataset_collection_setup}. For both the RGB and event datasets, manual ground truth (GT) annotation was carried out to facilitate tracker and classifier evaluation. 
In addition, the event and RGB data were made to have similar field-of-view (FoV) for a close comparison.
%Out of these, site 3 recordings were captured (shown in Fig.~\ref{PGP_loc}) for the performance comparison with simultaneously recorded frame-based data. %using a ZED stereo vision camera \cite{ZED} (setup shown in Fig~\ref{fig:Dataset_collection_setup}). 
%. report here the class size distributions

\textbf{Data Preparation for NNDC training: } As mentioned in Section~\ref{subsec:ebframegen}, events were aggregated at a frame rate of $15$ Hz ($t_F=66$ ms) to form 1B1C and 1B2C frames. We noted that the size of objects played a significant role for the NNDC model since an anchor box guides the class size. The objects at site 3 location had significantly different mean class sizes when compared to other sites (shown in Table~\ref{tab:class_sizes}). Therefore, to facilitate the model training, we rescaled the frame by half to $120\times90$ at site 3 location using nearest neighbor interpolation.


\begin{figure}[t]
\centering     %%% not \center
\includegraphics[width=70mm]{img/site_locations/experimental_setup_with_label.png}
 \caption{Experimental setup with ZED \cite{ZED} and DAVIS \cite{brandli2014240} mounted on custom-made 3D mount.}
\label{fig:Dataset_collection_setup}
\end{figure}


% Dataset collected by \ref{fig:Dataset_collection_setup} captured using ZED are crafted to create RGB frames with FoV30 and FoV90.The results obtained with frames with FoV 30 and FoV 90 are hereby refered as  SiamMask-RGB-FoV30 and SiamMask-RGB-FoV90 respectively.

% \begin{comment}
\begin{figure}
\centering
\subfloat[Site 1] {{\includegraphics[width=9cm]{img/site_locations/ENG.png}}\label{ENG_loc}}
\vspace{0.1em}
\subfloat[Site 2] {{\includegraphics[width=9cm]{img/site_locations/LT4.png}}\label{LT4_loc}}
\vspace{0.1em}
% \subfloat[Site  3] {{\includegraphics[width=9cm]{img/site_locations/YIH.png}}}
% \vspace{0.1em}
\subfloat[Site 3] {{\includegraphics[width=9cm]{img/site_locations/PGP.png}}\label{PGP_loc}}
\caption{Visual representation of datasets, i.e EBBI (Left) and RGB Image (Right), recorded at various sites discussed in Table \ref{tab:dataset_statistics_overview}}
\label{fig:Locations}
\end{figure}
% \end{comment}

%---------------------------------------------------------
Table~\ref{tab:dataset_statistics_overview} shows the statistical distribution of the dataset in terms of the number of samples obtained for each class category, and the number of recordings kept from each site for training and testing. The $42\times42\times2$ samples from the frames are obtained after applying CCL RP along with their correct positions, $BB_{conf}$ and class information, by matching the respective samples with interpolated GT annotations. We also randomly selected $\approx63,000$ noisy samples obtained from CCL RP that did not match with any GT annotations (with $IoU<0.1$) so that the network could classify them as a separate background class and give a predicted $\hat{BB}_{conf}$ to each less than $thr=0.1$. Assigning a different class was also necessary because these samples do not fit in any class category and in this class's absence, $Loss_1$ could not be optimized.

Note that we did not consider samples from pedestrians in the training data acquisition since they generate very few events due to their small size and slow speed. Simultaneous tracking of pedestrians and vehicles is kept as a future work. In total, we had $C=5$ with classes: background, car/van, bus, bike and truck in our model with a total of $C+5 = 10$ outputs. Since the buses and trucks were generally bigger than the size of $42\times42$, we also included cropped samples from top-left, top-right, bottom-left and bottom-right sections of their RPs. This helped to reduce the class-wise sample variance, and also provided the information from the object's frontal and posterior region for tuned BB prediction. The bikes were augmented by random rotation within $\pm$15 and translation by some random amounts within the fixed area of $42\times42$. The samples from recordings assigned for testing were also collected using the same criteria, but without any noisy samples having an $IoU<0.1$. The main objective of the training was to improve the $BB_{conf}$, increase the BB actual overlap with the object, and also report its correct class.

%-----------------------------------------------
% \begin{table}[t]
% \caption{Dataset statistics in detail.}
% \centering
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{tabular}{@{}|l|llll|@{}}
% \toprule
% S.No                                                                                                & {\color[HTML]{000000} Site 1}     & {\color[HTML]{000000} Site 2}      & {\color[HTML]{000000} Site 3}      & {\color[HTML]{000000} Site 4}     \\ \midrule
% {\color[HTML]{000000} Duration}                                                                     & {\color[HTML]{000000} 1h53m}      & {\color[HTML]{000000} 4h12m}       & {\color[HTML]{000000} 41m}         & {\color[HTML]{000000} 1h}         \\ \midrule
% {\color[HTML]{000000} Time}                                                                         & {\color[HTML]{000000} 3 PM, 4 PM} & {\color[HTML]{000000} 3 PM, 4 PM}  & {\color[HTML]{000000} 6:00 PM}     & {\color[HTML]{000000} 3:00 PM}    \\ \midrule
% {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}No.of \\ Events\end{tabular}}                   & {\color[HTML]{000000} 119107}     & {\color[HTML]{000000} 232678}      & {\color[HTML]{000000} 37612}       & {\color[HTML]{000000} 55373}      \\ \midrule
% {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}Train Test \\Split\end{tabular}} & {\color[HTML]{000000} 6 | 2}      & {\color[HTML]{000000} 6 | 3}       & {\color[HTML]{000000} 0 | 2}       & {\color[HTML]{000000} 2 | 1}      \\ \midrule
% {\color[HTML]{000000} Car/Van}                                                                      & {\color[HTML]{000000} 18232|379}  & {\color[HTML]{000000} 16918 | 382} & {\color[HTML]{000000} 23291 | 224} & {\color[HTML]{000000} 6514 | 211} \\ \midrule
% Bus                                                                                                 & {\color[HTML]{000000} 8081 | 165} & {\color[HTML]{000000} 8019 | 177}  & {\color[HTML]{000000} 1485 | 18}   & {\color[HTML]{000000} 1201 | 27}  \\ \midrule
% Bike                                                                                                & {\color[HTML]{000000} 1378 | 35}  & {\color[HTML]{000000} 1604 | 39}   & {\color[HTML]{000000} 2924 | 34}   & {\color[HTML]{000000} 512 | 22}   \\ \midrule
% Truck                                                                                               & {\color[HTML]{000000} 2256 | 47}  & {\color[HTML]{000000} 2513 | 56}   & {\color[HTML]{000000} 1075 | 10}   & {\color[HTML]{000000} 501 | 15}   \\ \bottomrule
% \end{tabular}

% \label{tab:dataset_statistics_overview}
% \end{table}
%------------------------------


\textbf{Training Details: }NNDC model was trained on $80\%$ of the training data randomly selected, while the rest was kept for validation. The model was trained on an NVIDIA TITANX GPU in the form of randomly shuffled batches of $128$ with $20$ assigned epochs, a learning rate of $0.01$ and $\lambda=5$. This model, trained using Adam optimizer with default hyperparameters, was written in Keras framework because of the ease of writing custom loss functions like equation~\ref{eq:lossfn}. Further, the overall unbalanced accuracy metrics on validation data after each epoch were used for early stopping of the training with patience $3$. The best model was saved for evaluation on the test recordings collected at different times. 

\textbf{Testing: }Table~\ref{tab:DAVIS_scores} shows the per-sample as well as per-track accuracies on all the test recordings, including overall balanced and unbalanced accuracies. As expected, per track accuracies are higher due to the majority voting, and in the case of the Bike category, it is possible to get $100\%$ classification performance. We attribute this  to the unique size and shape of the bikes relative to the other categories. Overall, the balanced accuracy closely trails the unbalanced accuracy, which implies the classifier makes sound judgements instead of skewed decisions caused by the unbalanced DAVIS dataset. 

%Next, we report the detection performance of the proposed blocks on the captured events dataset, followed by comparison to existing works such as SiamMask using both the events and the RGB datasets.

% \begin{table}[]
% \caption{Classification Scores for DAVIS sensor testing videos}
% \centering
% \begin{tabular}{lll}
% \hline
% {\color[HTML]{000000} \textbf{Class Categories}} & {\color[HTML]{000000} \textbf{per Sample scores}} & {\color[HTML]{000000} \textbf{per Track scores}} \\ \hline
% {\color[HTML]{000000} Car/Van} & {\color[HTML]{000000} 86.49} & {\color[HTML]{000000} 94.76} \\
% {\color[HTML]{000000} Bus} & {\color[HTML]{000000} 92.57} & {\color[HTML]{000000} 97.01} \\
% {\color[HTML]{000000} Bike} & {\color[HTML]{000000} 75.71} & {\color[HTML]{000000} 100} \\
% {\color[HTML]{000000} Truck} & {\color[HTML]{000000} 51.4} & {\color[HTML]{000000} 73.33} \\ \hline
% {\color[HTML]{000000} \textbf{Overall Unbalanced}} & {\color[HTML]{000000} \textbf{85.68}} & {\color[HTML]{000000} \textbf{94.33}} \\
% {\color[HTML]{000000} \textbf{Overall Balanced}} & {\color[HTML]{000000} \textbf{76.54}} & {\color[HTML]{000000} \textbf{91.28}} \\ \hline
% \end{tabular}
% \label{tab:class_scores}
% \end{table}
% %----------------------------------------------------
\begin{table}[H]
\caption{Classification accuracies for testing samples recorded using DAVIS}
\centering

\begin{tabular}{lcc}
\hline
{\color[HTML]{000000} \textbf{Category}} & {\color[HTML]{000000} \textbf{per sample (\%)}} & {\color[HTML]{000000} \textbf{per track (\%)}} \\ \hline
{\color[HTML]{000000} Car/Van} & {\color[HTML]{000000} 86.59} & {\color[HTML]{000000} 95.8} \\
{\color[HTML]{000000} Bus} & {\color[HTML]{000000} 89.81} & {\color[HTML]{000000} 98.1} \\
{\color[HTML]{000000} Bike} & {\color[HTML]{000000} 81.02} & {\color[HTML]{000000} 100} \\
{\color[HTML]{000000} Truck} & {\color[HTML]{000000} 53.39} & {\color[HTML]{000000} 76.92} \\ \hline
{\color[HTML]{000000} \textbf{Unbalanced accuracy}} & {\color[HTML]{000000} \textbf{85.07}} & {\color[HTML]{000000} \textbf{95.39}} \\
{\color[HTML]{000000} \textbf{Balanced accuracy}} & {\color[HTML]{000000} \textbf{77.70}} & {\color[HTML]{000000} \textbf{92.70}} \\ \hline
\end{tabular}
\label{tab:DAVIS_scores}
\end{table}

\begin{figure*}[t]
%%% not \center
\resizebox{\textwidth}{!}{
\begin{tabular}{ccc}
\subfloat[]{\includegraphics[width=.33\textwidth]{img/plots/filteringComparison_r.png}} &
\subfloat[]{\includegraphics[width=.33\textwidth]{img/plots/rpComparison_r.png}} &
\subfloat[]{\includegraphics[width=.33\textwidth]{img/plots/TrackerPerfComparison_r.png}}
\end{tabular}
}
 \caption{(a) Comparison between Event based filtering (Refractory Filter + NN-Filter + EBBI) Vs. Median Filtering (EBBI + Median Filter) followed by CCL RP showing comparable performance with event based filtering slightly superior. (b) Comparison between different RP methods showing NNDC (CCL+NNDC) to be much superior than others in a EBBI+RP setup. (c) Comparison between trackers show EBBINNOT to be best in terms of weighted F1-Score.}
\label{fig:filtering_RP_track_Comparison}
\end{figure*}
\subsection{Median filtered EBBI vs. Event-based AER noise filtering}
\label{subsec:Noise_Filtering_Comparison}
To evaluate the effect of the proposed median filtering approach on the detection performance of the whole pipeline, we replaced it with the commonly used AER event-based nearest neighbour filtering approach \cite{fnins2018, RameshFrontiers, RameshDARTIEEE}. For a fair comparison, a refractory period of $5ms$ in a neighbourhood of $3\times3$ was implemented for the event filtering approach, similar to the $3\times3$ window used for the proposed median filtering approach. Since our proposed median filter with EBBI gives on par performance with the event-based filtering approach, as shown in Figure~\ref{fig:filtering_RP_track_Comparison}(a), we advocate it for low-power hardware implementations as carried out in this work. 
%In other words, the two methods are comparable and median filtering results in no major degradation of information for detection, classification and tracking.



% \begin{figure}[t]
% \centering     %%% not \center
% \includegraphics[width=9cm]{img/plots/filteringComparison.png}
%  \caption{Weighted F1 scores for Event Stream + Refractory Filter + NN-Filter Vs. EBBI + Median Filter followed by CCL}
% \label{fig:filteringComparison}
% \end{figure}

% \captionsetup[table]{labelformat=empty}
%\begin{figure}[]
%\scriptsize
%    \centering
%  \begin{tabular}{@{}c@{}}
 %   \includegraphics[width=9cm]{img/plots/filteringComparison.png} \\[\abovecaptionskip]
 % \end{tabular}
%\begin{tabular}{|c|c|c|}
 %               \hline
 %               Curve Name & EBBI+Hist RP & EventFiltering+EBGI+CCL \\ \hline
 %               AUC & 0.2122 & 0.2321 \\ \hline
%\end{tabular}

 %   \caption{Weighted F1 scores for Event Stream + Refractory Filter + NN-Filter Vs. EBBI + Median Filter}
%    \label{fig:filteringComparison}
%\end{figure}

\subsection{Comparison of Region Proposal Networks}% is this heading correct
In order to pick the best region proposal for the proposed pipeline, we ran the three RPNs, namely HIST, CCL and CCL + NNDC RP on the test dataset while restricting the maximum RPs to eight per frame. In this evaluation, the greedy NMS in NNDC had $thr^{ns}=0.3$ for suppressing the boxes. To compare the performance at different $IoUs$, we used ground truth annotations at the same timestamps corresponding to the RPs. 
\par
Figure~\ref{fig:filtering_RP_track_Comparison}(b) shows the weighted F1 scores for the different RPs. Overall, the proposed CCL+NNDC RP significantly outperforms other RPs, as shown in Figure~\ref{fig:filtering_RP_track_Comparison}(b) with higher area under curve (AUC), calculated using trapezoidal numerical integration. Interestingly, HIST RP performs better than CCL RP by itself, due to lesser fragmentation by merging of overlapping regions. Integrating NNDC after CCL significantly improves this performance. Therefore, we adapt CCL+NNDC RP as part of our proposed pipeline and is also referred as hybrid RP.
%It is clear that CCL + NNDC RP is considerably better than the other two RPs with higher area under curve (AUC). 
%Nonetheless, to counter-check a possible scenario that CCL with the tracker might be able to perform better, we also compared its performance with CCL + NNDC RP by introducing OT and KF trackers. Figure~\ref{fig:cclToNNDCImprovement} shows that CCL with different trackers still fails completely as compared to CCL + NNDC RP even at higher $IoUs$.

\subsection{Comparison of Tracker}
\label{sec:flowcompare}
For the purpose of fair comparison of performance of different trackers, we ensured that the same region proposal network, tracker parameters, tracker log generation method and evaluation metrics were used. For comparison of KF-Tracker and OT, the number of region proposals and trackers per frame were restricted to a maximum of $8$, the threshold for treating an object to be lost during tracking was set at invisibility for $5$ consecutive frames or less than $60\%$ visibility when the track is still valid. \textcolor{red}{While for EBMS, the events were filtered using a refractory layer with period of $50ms$, followed by NN-Filter with period of $5ms$. The minimum number of events required for cluster formation were kept $8$, maximum radius of cluster was kept $130$, and a time limit of $100ms$ was assigned in case of inactivity of cluster. These hyperparameter values were obtained after series of runs for optimization of EBMS.} Figure \ref{fig:exemplar_tracks} illustrates the sample tracks generated for different types of vehicles for the trained EBBINNOT pipeline. Based on the observations made in~\cite{Authorsbmvc19}, we excluded tracks for human class while calculating the F1-scores for all the $5$ test dataset recordings excluding site 3.

% \begin{figure}[t]
% \centering     %%% not \center
% \includegraphics[width=9cm]{img/plots/TrackerPerfComparison.png}
%  \caption{Weighted F1 scores for tracking in DAVIS recordings}
% \label{fig:Tracker_Performance_Comparison}
% \end{figure}

As shown in Figure \ref{fig:filtering_RP_track_Comparison}(c), it can be noted that OT performs slightly better than KF and significantly better than the purely event based EBMS tracker.
%\textcolor{red}{Need critical discussion on why -- for example, you did the ablation experiments by seeing which part of the OT code is responsible for most improvement} 
\input{04_results_OT_analysis}

%Thus, we track the RPs (generated by our hybrid RP) using overlap Tracker (OT) and this completes the pipeline of the proposed tracker. 
%\begin{figure}[]
%\scriptsize
%    \centering
%  \begin{tabular}{@{}c@{}}
%    \includegraphics[width=9cm]{img/plots/TrackerPerfComparison.png} \\[\abovecaptionskip]
%  \end{tabular}
%\begin{tabular}{|c|c|c|c|}
%                \hline
%                Curve Name & EBBI+CCL+NNDC+OT & EBBI+CCL+NNDC+KF & EBMS \\ \hline
%                AUC & 0.3938 & 0.3633 & 0.1920 \\ \hline
%\end{tabular}
%    \caption{Weighted F1 scores for tracking in DAVIS recordings}
%   \label{fig:davisF1}
%\end{figure}

\begin{figure*}
\centering
\resizebox{\textwidth}{!}{
\includegraphics[]{img/trackImage.png}
}
\caption{Exemplar detection and classification results from the described EBBINNOT pipeline for tracks of different vehicles.}
\label{fig:exemplar_tracks}
\end{figure*}

\subsection{Comparison to state-of-the-art } 
\label{sec:statecompare}
In this section, we report the performance of the proposed EBBINNOT compared to the frame-based state-of-the-art tracker, namely SiamMask, and event-based state-of-the-art approach EBMS. %We report the data collection and preparation process, which involves recording both event and RGB data simultaneously at site 3 shown in Figure \ref{fig:Locations}. 
Since $2/3^{rd}$ of data recorded at site 3 was used to train NNDC model, as stated in Table \ref{tab:dataset_statistics_overview}, we used remaining $1/3^{rd}$ of data for evaluation. Note that original RGB dataset with FoV $90^\circ$ is used as input to SiamMask and corresponding output is referred as SiamMask-RGB in this section.
%Finally, we show the performance of our proposed EBBINNOT compared to EBMS on event-based data and SiamMask on RGB data. 


%\subsubsection{Evaluation for SiamMask}
%SiamMask \cite{DBLP:Siammask} is inspired from that great success of fully convolution Siamese trackers \cite{DBLP:FC-SiameseNetworks} in object tracking . Unlike others, Siam Mask solely relies on initial bounding box coordinates of object in the first frame of test video and estimates object position and segmentation mask in consecutive frames. Apart from establishing new state of art on VOT-2018, Siam Mask is also popular for its simplicity (adaptable to new test environment) and fast speed. However, Siam Mask fails to perform in case of motion blur and no object instances in particular frame.  
    
%\textbf{Why SiamMask tracking with event-based data?}
 

\par

\begin{figure}[t]
\scriptsize
\centering
\includegraphics[width=9cm]{img/plots/SOTAPerfComaprison_r.png} 
\caption{Comparison of the proposed EBBINNOT, SiamMask \cite{DBLP:Siammask} and Event-Based Mean-Shift (EBMS) \cite{delbruck2013robotic}}
\label{fig:SiamMaskcomp}
\end{figure}
Figure~\ref{fig:SiamMaskcomp} shows the weighted F1 scores at various $IoU_{th}$ for 5 test recordings excluding site 3. 
%It is clear that our proposed tracker outperforms both the state-of-the-art methods. 
We observed that SiamMask was not able to match the performance of EBBINNOT due to its inherent use of similarity matching, which failed under occlusion scenarios. In other words, SiamMask fails to perform in scenarios where vehicles pass each other, as illustrated in Figure \ref{fig:SiamMask_Overlap_Sequence}. The other factor contributing to SiamMask's poor performance was that the background road markings and footpath patterns of the scene became part of the object representation as shown in Figure \ref{fig:SiamMask_Latching}, causing missed tracks. 

% \begin{comment}

\begin{figure}[t]
\centering
\subfloat[Occlusion scenario.] {\includegraphics[width=9cm]{img/SiamMask_overlap_sequence.png}
\label{fig:SiamMask_Overlap_Sequence}}
\vspace{0.1em}
\subfloat[Background noise I.] {\includegraphics[width=9cm]{img/SiamMask_latching_scenario.jpg}
\label{fig:SiamMask_Latching}}
\vspace{0.1em}
\subfloat[Background noise II.]
{\includegraphics[width=9cm]{img/plots/SiamMask_Initialization_scenario.jpg}
\label{fig:SiamMask_Initialization_Scenario}}
\caption{Tracking performance of SiamMask under challenging scenarios. It fails to track either to background road markings or occluding objects becoming part of its online object learning representation.}
\label{fig:SiamMask_failed_cases}
\end{figure}


%the object representation and are responsible for missed tracks 
%of the scene that caused missed tracks, which became part of the object representation, as shown in Figure \ref{fig:SiamMask_Latching}.
%w.r.t track length for SiamMask-RGB-FoV30 than SiamMask-RGB-FoV90, which  As both work in favour of event data which leads to SiamMask-Events outperforming SiamMask-RGB methods.
\par
%\vspace{0.1em}
%\begin{figure}[t]
%\centering     %%% not \center
%\includegraphics[width=80mm]{img/PGP_EventsBasedMethods_Gen_FoV.png}
%\vspace{0.1em}
%\subfloat[]{\includegraphics[width=80mm]{images/FR1.eps}}
 %\caption{Comparison of the proposed tracker, SiamMask \cite{DBLP:Siammask}, Event-Based Mean-Shift (EBMS) \cite{Delbruck2013} in terms of F1 score at different IoU thresholds.}
%\label{fig:SiamMaskcomp}
%\end{figure}

Overall, our proposed tracker outperforms the multi-object EBMS tracker and SiamMask. In spite of this good performance, it was noticed that on re-scaling the frame size by half to $120\times90$ at site 3 location, as previously noted in Section \ref{subsec:Experiments-on-DAVIS}, the NNDC model did not always pick the right size for individual classes. This minor drawback remains to be addressed in future works using techniques such as transfer learning.

%\subsubsection{Comparison of Tracker performance with SiamMask \cite{DBLP:Siammask} using RGB image data} 

%While the comparison between these two modalities is indirect, it shows the performance of the tracking and classification modules under the same data capturing scenario.

\subsection{Computational Cost}
\label{subsec:Computational_Cost}

\begin{table}[t]
\centering
\caption{Computational Count Estimation: $C_{KF}$ Vs. $C_{OT}$}
\begin{tabular}{ccccc}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Recording\\ Site\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}No. of\\ Recordings\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}OT\\ Estimate\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}KF\\ Estimate\end{tabular}} & \textbf{KF:OT} \\
\hline
Site 1             & 4                     & 119                   & 698                   & 6              \\
Site 2             & 4                     & 351                   & 2472                  & 7              \\

\hline
\textbf{Average}            & \textbf{8 Recordings}                     & \textbf{235}                   & \textbf{1585}                  & \textbf{6.5}\\
\hline
\end{tabular}
\label{tab:trackerComputes}
% \FloatBarrier
\end{table}

The average number of computations per frame performed by KF-Tracker ($C_{KF}$) and OT ($C_{OT}$) were estimated using eq.~\ref{eq:KF} and eq.~\ref{eq:OT} respectively, and these results were verified to be close to the actual computation count obtained by incrementing a counter with count weighted by computations in a step at run time, with an error margin of $\pm0.01\%$. As shown tabulated in Table \ref{tab:trackerComputes}, KF-Tracker performs $\approx6.5\times$ more computations averaged across $8$ recordings at $2$ sites as compared to the OT.

\par
Based on the SiamMask architecture presented in \cite{DBLP:Siammask}, computations and memory usage are calculated layer-by-layer and then summed considering all network parameters and input dimensions. Total computations and memory requirements were deduced to be $\approx38000M$ operations per frame and $\approx 157MB$ respectively.

\par
It is already known from Section~\ref{sec:NNDCrp} that EBBINN has a computes bound of $\approx17.3M$ operations per frame and since OT does not add much computes, SiamMask uses $\approx2200\times$ more computes per frame and demands $\approx1450\times$ more memory than EBBINNOT, due to its Siamese-based deep neural network architecture. Therefore, EBBINNOT offers a fair advantage in terms of total computation and memory usage.

\par
%The authors in~ derived the formula for 

The total number of computes per frame ($C_{EBMS}$) and the memory requirement in bits ($M_{EBMS}$) for the EBMS \cite{AuthorsEBBIOT} algorithm are given by,
\begin{align}
\label{eq:EBMS}
    C_{EBMS} =& \overline{N}\times [9~\overline{CL}^2+{(169+16~\gamma_{merge})}~\overline{CL} +11]\notag\\
    M_{EBMS} =& 408 CL_{max}+ 56,
\end{align}
respectively, where $\overline{N}$ is the average number of events per frame, $\overline{CL}$ is the average number of active clusters at any given time ($\approx \overline{N_T}$), $\gamma_{merge}$ is the probability of two clusters merging, and $CL_{max}$ is the maximum number of potential clusters. Assuming the past $10$ positions of cluster for the current velocity calculation, $CL_{max}=8$ and for our dataset, $\overline{CL}\approx 2$, $\gamma_{merge}\approx0.1$ and $\overline{N}\approx 650$, EBMS requires 252 kops per frame which is $\approx68\times$ lower than EBBINNOT, and a memory of $3.32$kB, which is nearly negligible. 

The proposed EBBINNOT, however,  significantly outperforms EBMS as shown in Figure \ref{fig:SiamMaskcomp}. This performance gain comes at the cost of slightly higher computations and memory usage. Overall, out of the three approaches considered here, EBBINNOT offers the best trade off between performance and computational complexity.
 %Note that \ref{fig:SiamMaskcomp} shows that EBBINNOT out performs EBMS by significant margin. Therefore, EBBINOT is preferred to EBMS. 

% --------------------------------------
%------------------------------



==> 05_01_tracks_figtex.tex <==
% \begin{figure*}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{ccccc}
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Car/image_1153.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Car/image_1162.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Car/image_1171.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Car/image_1180.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Car/image_1189.png}}\\
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Bus/image_1661.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Bus/image_1670.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Bus/image_1680.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Bus/image_1691.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Bus/image_1704.png}}\\
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Bike/image_4906.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Bike/image_4913.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Bike/image_4920.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Bike/image_4927.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Bike/image_4934.png}}\\
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Truck/image_8650.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Truck/image_8659.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Truck/image_8666.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Truck/image_8675.png}} &
% \subfloat[]{\includegraphics[width = 1.5in]{img/tracks_fig/Truck/image_8684.png}}
% \end{tabular}
% }
% \caption{4 x 5}
% \end{figure*}




% \begin{figure*}
% \centering
% % \begin{subfigure}
% \subfloat[Car/Van Track]{
% \resizebox{\textwidth}{!}{
% % \begin{tabular}{ccccc}
% % \subfloat[]{
% \includegraphics[width = 1.5in]{img/tracks_fig/Car/image_1153.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Car/image_1162.png}
% \includegraphics[width = 1.5in]{img/tracks_fig/Car/image_1171.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Car/image_1180.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Car/image_1189.png}
% % }\\

% % \end{tabular}

% }
% } \\\vspace*{-0.9em}
% \subfloat[Bus Track]{
% \resizebox{\textwidth}{!}{
% % \begin{tabular}{ccccc}

% % \subfloat[]{
% \includegraphics[width = 1.5in]{img/tracks_fig/Bus/image_1661.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Bus/image_1670.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Bus/image_1680.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Bus/image_1691.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Bus/image_1704.png}
% % }\\

% % \end{tabular}
% }
% }\\\vspace*{-0.9em}
% \subfloat[Bike Track]{
% \resizebox{\textwidth}{!}{
% % \begin{tabular}{ccccc}
% \includegraphics[width = 1.5in]{img/tracks_fig/Bike/image_4906.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Bike/image_4913.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Bike/image_4920.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Bike/image_4927.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Bike/image_4934.png}

% % \end{tabular}
% }
% }\\\vspace*{-0.9em}
% \subfloat[Truck Track]{
% \resizebox{\textwidth}{!}{
% % \begin{tabular}{ccccc}
% \includegraphics[width = 1.5in]{img/tracks_fig/Truck/image_8650.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Truck/image_8659.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Truck/image_8666.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Truck/image_8675.png} 
% \includegraphics[width = 1.5in]{img/tracks_fig/Truck/image_8684.png}
% % }\\

% % \end{tabular}
% }
% }
% % \end{subfigure}
% \caption{Exemplar detection and classification results from the described pipeline}
% \label{fig:exemplar_tracks}
% \end{figure*}


==> biography.tex <==

\begin{IEEEbiographynophoto}
{Vivek Mohan}
(S’ 14) received his B.Tech. degree in Electronics and Communication Engineering from JNTU - Hyderabad in 2016 and Joint M.Sc. in Integrated Circuit Design from Technical University of München and Nanyang Technological University (NTU) Singapore in 2019. After graduation, he worked as a Research Associate in the BRAIN Systems Lab - CICS, NTU in the area of neuromorphic vision. Vivek is currently a Ph.D. candidate at the School of Electrical and Electronic Engineering, NTU. His research interests include integrated circuit design, neurotechnology and neuromorphic engineering.
\end{IEEEbiographynophoto}
\vspace{-1 cm}
\begin{IEEEbiographynophoto}
{Deepak Singla}
(M’ 20) received his B.Tech in Electrical Engineering (Power \& Automation) from the Indian Institute of Technology, Delhi in 2018. After the graduation, he joined Nanyang Technological University, Singapore as a Project Officer in the BRAIN Systems Lab - CICS headed by Dr. Basu. Since then, he is working on IoT based applications of neuromorphic vision sensors and designing low computational cost and reliable systems for the same. His research interests include neurmorphic engineering, brain-machine intelligence and computer vision. 
\end{IEEEbiographynophoto}
\vspace{-1 cm}
\begin{IEEEbiographynophoto}
{Tarun Pulluri}
received his B.Tech degree in Electronics and Communications Engineering from JNTUH College of Engineering Hyderabad and M.Enng degree in Microelectronics and Embedded Systems from Asian Institute of Technology (AIT) in 2018. After graduation, he joined AIT - AI Center as a research assistant. He is currently working as a research attachment in the Neuromorphic lab at the National University of Singapore. His research interests include deep learning, computer vision, computational neuroscience, neuromorphic engineering, and robotics.
\end{IEEEbiographynophoto}
\vspace{-1 cm}
\begin{IEEEbiographynophoto}
{Andres Ussa}
received his B.Sc. degree in Mechatronics Engineering from Nueva Granada Military University in 2012 and Joint M.Sc. in Embedded Computing Systems from TU Kaiserslautern and University of Southampton in 2016. His previous research experience has been focused on embedded systems design and machine learning applications. He had a short experience as a Software/Hardware Developer for consumer electronics. 
\end{IEEEbiographynophoto}
\vspace{-1 cm}
\begin{IEEEbiographynophoto}
{Pradeep Kumar Gopalakrishnan}
(M’ 01, SM' 08) received his B.Tech. degree in Electrical Engineering from the University of Kerala, Trivandrum, India (1989) and his M.Tech. degree in Electronics Design and Technology from the Indian Institute of Science, Bangalore, India (1997). He has more than 25 years of experience in ASIC and embedded systems design, at companies such as Philips Semiconductors (Singapore), Broadcom (Singapore), Institute of Microelectronics - A*STAR (Singapore), Siemens Corporate Research (Bangalore, India) and Xilinx (Hyderabad, India). He is currently a researcher and part-time Ph.D student at Nanyang Technological University, Singapore. His research interests include low-power Machine Learning architectures and Neuromorphic systems.
\end{IEEEbiographynophoto}
\vspace{-1 cm}
\begin{IEEEbiographynophoto}
{Bharath Ramesh}
received the B.E. degree in Electrical \& Electronics Engineering from Anna University of India in 2009; M.Sc. and Ph.D. degrees in Electrical Engineering from National University of Singapore in 2011 and 2015 respectively, working at the Control and Simulation Laboratory on Image Classification using Invariant Features. Dr. Bharath is a Lecturer at Western Sydney University with extensive experience in the broad area of Pattern Analysis and Machine Vision. Over the past decade, he has worked on diverse projects, ranging from theoretically oriented research for visual object recognition to practical neuromorphic systems for traffic surveillance. At present, his research is centered on distributed neuromorphic systems and pattern recognition.
\end{IEEEbiographynophoto}
\vspace{-1 cm}
\begin{IEEEbiographynophoto}
{Arindam Basu}
(M’ 10, SM' 17) received the B.Tech and M.Tech degrees in Electronics and Electrical Communication Engineering from the Indian Institute of Technology, Kharagpur in 2005, the M.S. degree in Mathematics and PhD. degree in Electrical Engineering from the Georgia Institute of Technology, Atlanta in 2009 and 2010 respectively. Dr. Basu received the Prime Minister of India Gold Medal in 2005 from I.I.T Kharagpur. He joined Nanyang Technological University in June 2010 and currently holds a tenured Associate Professor position.

He is currently an Associate Editor of IEEE Sensors journal, IEEE Transactions on Biomedical Circuits and Systems and Frontiers in Neuroscience. He was a Distinguished Lecturer for IEEE Circuits and Systems Society for the 2016-17 term. Dr. Basu received the best student paper award at Ultrasonics symposium, 2006, best live demonstration at ISCAS 2010 and a finalist position in the best student paper contest at ISCAS 2008. He was awarded MIT Technology Review's inaugural TR35@Singapore award in 2012 for being among the top 12 innovators under the age of 35 in SE Asia, Australia and New Zealand. His research interests include bio-inspired neuromorphic circuits, non-linear dynamics in neural systems, low power analog IC design and programmable circuits and devices.
\end{IEEEbiographynophoto}



==> random_learning_algorithms.tex <==
\section{Learning Algorithms}
\label{sec:learning_algorithms}

In this section, we review some of the most popular learning algorithms that have been implemented on neuromorphic hardware. In some cases, modifications to the original algorithm have been proposed to make it feasible to implement on low-precision platforms with only locally available information. Most recent work has focussed on spike based learning rules while only a few have considered non-spike based ones\cite{soul_chetan,fg_holleman}. Hence, we discuss the spike based rules in details while summarizing the non-spike based ones. 

Before going into details, let us review some of the desirable properties of the algorithms.
\begin{itemize}
\item \textbf{Computational complexity} i.e number of operations needed per weight update should be low.
\item \textbf{Locality} of the weight update rule is desired. In other words, the weight update rule should ideally only need information related to the variables in the computational element (neuron) connected to it.
\item \textbf{Convergence speed} of the algorithms should be as fast as possible.
\end{itemize}


\begin{figure}[!t]
\centerline
{\includegraphics[width=0.35\textwidth]{stdp_theory.PNG}}
\caption{Theoretical model of weight change as a function of time difference of pre- and post-synaptic spikes in STDP\cite{roshan_triplet}.}\label{fig:stdp_theory}
\end{figure}

\subsection{Least Mean Square (LMS), Perceptron}
\label{sec:lms}
Two of the oldest learning rules derived for non-spiking networks were the LMS and the Perceptron learning rules\cite{widrow_review}. They were typically used to train single layer neural networks. Both rules follow the so-called ``Minimum Disturbance Principle'' \cite{widrow_review} that aims to correct the error at every step by minimal change in parameters to maximize memory capacity.

\subsubsection{LMS}
The simple neural network under consideration here is called the Adaptive Linear Combiner (ADALINE) and is described by the following equations:
\begin{align}
\label{eq:adaline}
s=\overline{X}^T\overline{W}\\
e=d-s
\end{align}
where $\overline{X_k}$ denotes the input vector, $\overline{W}$ is the weight vector, $d$ is the desired output and $e$ is the corresponding error. In this case, the LMS learning rule prescribes a weight update \cite{widrow_book} as given by:
\begin{align}
\label{eq:lms}
\overline{\Delta W}=\alpha\frac{e\overline{X}}{\vert \overline{X} \vert ^2}
\end{align}
where $\alpha$ is typically chosen to be between $0.1$ and $1$ for a good tradeoff between stability and convergence speed. It can be shown that the error reduces at every step at a fixed rate dependent on $\alpha$. This rule is known to minimize mean squared error. The LMS algorithm has often been implemented in adaptive circuits especially for filters\cite{fg_app2,fg_app7}.

\subsubsection{Perceptron}
In this case, we consider a non-linear network by adding a threshold function at the output of the ADALINE. The new output $y=sgn(s)$ where $sgn()$ is the signum function\cite{widrow_review}. The new error is now  defined as $e=d-y$. Then, the perceptron weight update\cite{rosenblatt_book} is given by:
\begin{align}
\label{eq:perceptron}
\overline{\Delta W}=\alpha\frac{e}{2}\overline{X}
\end{align}
Here, $\alpha$ does not affect stability but only affects rate of convergence. The perceptron rule is guaranteed to converge to classification error of $0$ if the patterns presented to it are linearly separable. However, for non-linearly separable patterns, the algorithm does not guarantee low classification errors. Other variants of this rule including margin \cite{mays_thesis} have also been proposed.

\subsection{Backpropagation and variants}
\label{sec:backprop}
Backpropagation and gradient descent have been the most popular learning algorithms for training both shallow and deep neural networks for past decades. It is simple, intuitive and works well for most of the real world applications. In standard gradient descent backpropagation, the error signal is backpropagated from output layer to the deeper layers on a neuron-by-neuron basis\cite{lillicrap2016random}. Mathematically, the output of layer $i$ of a neural network, $\overline{h_i}$ is given by:
\begin{equation}
\label{forward_pass}
\overline{h_i}=f(W_{ij}\overline{h_j}+\overline{b_i})
\end{equation}
where $W_{ij}$ is the weights connecting layer j and layer i, $\overline{b_i}$ is the bias and $f(.)$ is the non-linear activation function. The weight update $\Delta W_{ij}$ is given by:
\begin{equation}
\label{backward_pass_1}
\Delta W_{ij}= -\eta \frac{\partial \overline{E}}{\partial W_{ij}}
\end{equation}
where $\eta$ is the learning rate and $\overline{E}$ is the error at the output layer.

In spite of the huge success of backpropagation in different forms of neural networks, several issues have been pointed out over the years regarding its hardware implementation and biological plausibility. Typical implementation of backpropagation necessitate use of high precision weights and smooth activation functions (tanh, sigmoid etc.) as well as a significant number of multiply and accumulate (MAC) operations for both forward and backward pass. From a hardware perspective, these features make backpropagation costly, both in terms of memory and power. Moreover, backpropagation requires global information about the errors well as weights in backward pass that are exactly symmetric with respect to the weights in the forward pass. This weight transport problem \cite{grossberg1987competitive}, along with  alternating forward and backward passes and precise floating point weights make standard backpropagation an implausible learning technique for brain as well as neuromorphic architectures \cite{neftci2017event}.

A proposed solution to reduce the computational complexity and optimize memory resources is the use of pipelined backpropagation \cite{mostafa2017hardware} and binary state network \cite{hubara2016binarized}. In binary state network, the output of a neuron can be unipolar (0/1) or bipolar (-1/1) binary. This modification transforms the MAC operations in the forward pass to simple additions and subtractions. In \cite{mostafa2017hardware}, error ternarization was proposed which removes the requirement of MAC operations even in the backward pass. Thus, all the network operations become equivalent to synaptic operations (SynOps) which can facilitate efficient neuromorphic implementations. In pipelined backpropagation, the network has access to the previous network states and therefore, can perform delayed weight updates during the subsequent forward pass without the need for an explicit backward pass. This architecture reduces the number of memory fetches and lookups (corresponding to backward pass) significantly. The reduction of redundant off-chip memory fetches can also reduce the power overhead appreciably \cite{mostafa2017hardware}.

Another significant constraint regarding hardware implementation of neural networks is the requirement of high precision floating point weights and gradients. This problem is addressed by two approaches: (1) off-chip learning using high resolution weights and gradients and consequently rounding off the weights to lower resolution for on-chip implementation and (2) on-chip learning using low resolution weights. In \cite{muller2015rounding} randomized rounding has been used to map high resolution gradients to low resolution discrete values. Moreover, k-means clustering has been used to map high resolution weights to low resolution values. One of the significant low resolution learning methods for on-chip learning is randomized unregulated step descent (RUSD) introduced in  \cite{muller2017randomized}. This method combines unregulated step descent (USD) with randomized rounding i.e. the step size for weight update is large (low resolution) but the weight update probability is low. So, the overall average weight update is small (comparable to high resolution weight update case).

A simple yet elegant solution has been proposed in \cite{lillicrap2016random} to solve the weight transport and global information problem of the backpropagation algorithm. In the proposed random backpropagation (RBP), the errors are backpropagated through a random weight matrix(B)  instead of the transpose of forward pass weights ($W^T$). So, the error update formula changes from $\Delta W\propto -W^Tex^T$ to $\Delta W\propto Bex^T$. Therefore, RBP is spatially and temporally local \cite{neftci2017event} and absence of feedback weight constraints makes it possible for a feedback architecture consisting of a separate feedback channel which is biologically more plausible. A possible explanation as to why this architecture works, is that the network weights adjust themselves to the random feedback weights and learns afterwards. 
\begin{table*}[h!]%[htbp]
\centering
\caption{Comparison of Learning Algorithms used in Recent Neuromorphic Machine Learning Systems}
\label{tab:algo_comparison}
 \begin{threeparttable}
\begin{tabular}{@{}cp{1.3cm}p{1cm}p{1cm}p{1.6cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}@{}}
\toprule
Ref     & Algorithm & Mode      & Type          & Accuracy & Precision (wt, internal) &Complexity& Locality&Convergence                                                                     \\ \midrule
 \cite{brader_sdsp} & SDSP & Spike     & Semi-supervised             & 96.5\% (MNIST) \tnote{a}           &   1-bit, high  &  Medium                         &  Local&Problem Specific                                                   \\
\cite{struct_frontiers} & Struct. plasticity & Spike     & Supervised             & 96.4\% (MNIST) \tnote{b} {2}           &   1-bit, high  & Medium                      &Global    & Slow                                             \\
\cite{diehl_cook} & STDP & Spike     & Un-supervised             & 95\% (MNIST) \tnote{c}           &   High  &    Low                      &  Local& Problem Specific                                             \\
\cite{struct_shaista_neco} & Struct. plasticity & Non-Spike     & Supervised             & 96/75/89\% (UCI)  \tnote{d}           &   1-bit, high    &     Medium                   & Global&Slow \\
       \cite{mostafa2017hardware} & Backprop (Pipelined) & Non-Spike     & Supervised             &  98.07\% (MNIST)\tnote{e}           &   8-bit, 2-bit &    High                       &Global& Medium \\
\cite{muller2017randomized} & Backprop (RUSD) & Non-Spike     & Supervised             & 76\%(CIFAR-10) 97.5\% (MNIST) \tnote{f}          &   7-bit, 1-bit  &   Medium                       & Global & Slow
       \\
       \cite{baldi2016learning} & Backprop (RBP) & Non-Spike     & Supervised             & 75\%(CIFAR-10) 96\% (MNIST)   \tnote{g}        &   High, high &  High                         & Global &Slow
     \\
\cite{neftci2017event} & Backprop (eRBP) & Spike     & Supervised             &  98\% (MNIST)\tnote{h}          &   High, high &  high                         & Local&Slow \\
       
\cite{soul_chetan} & LMS (SOUL) & Non-spike & Supervised & 95\% (MNIST)\tnote{i}  & 15-bit, 15-bit & Low & Global & Fast. \\

\bottomrule
\end{tabular}
\begin{tablenotes}
\item[a] SDSP is unsupervised but has been applied in this reference with a supervisory teacher signal. Internal variable is analog and precision requirement not specified. $115$ neurons with $\approx 117K$ synapses used.
\item[b] Neurons with dendritic nonlinearity used. Internal variable is analog and precision requirement not specified. $100$ neurons with $3960$ dendrites and $\approx 20K$ synapses used.
\item[c] $6400$ neurons with $\approx 500K$ synapses used. Adaptive threshold and conductance based models used.
\item[d] Accuracies reported on BC, Heart and Ion datasets from UCI repository.\cite{uci}
\item[e] 2 hidden layers with 600 neurons each
\item[f] BinaryNet \cite{courbariauxbinarynet} with RUSD for CIFAR-10 and a CNN (2 conv. layers with 256 neurons each, 2 maxpooling layers and a fully connected layer) with RUSD for MNIST.
\item[g] CNN (3 conv. layers with 64 neurons each, 3 max-pooling layers and a fully connected layer) with random backprop for CIFAR-10 and a DNN with 4 hidden layers (100 neurons each) for MNIST.
\item[h]  2 hidden layers with 500 hidden nodes each
\item[i] $16,384$ hidden neurons used, trained for 3 epochs of $60,000$ training images.
\end{tablenotes}
\end{threeparttable}
\end{table*} 
The RBP has also  shown promise in spiking neural networks (event-driven RBP or eRBP)\cite{neftci2017event} and deep networks \cite{baldi2016learning} on datasets such as MNIST, CIFAR-10, etc. Several variants of this algorithm have also been proposed such as skipped random backpropagation (SRBP), adaptive random backpropagation (ARBP), and adaptive skipped random backpropagation (ASRBP)~\cite{baldi2016learning}.

\subsection{Spike Timing Dependent Plasticity (STDP)}
\label{sec:stdp}
By far, the most popular learning algorithm to be implemented in recent adaptive neuromorphic systems is spike time dependent plasticity (STDP)\cite{stdp_review1,stdp_review2}. STDP has been widely observed in experiments\cite{stdp_measure1,stdp_measure2} as well as used in computational models\cite{stdp_app1,stdp_app2}. One popular mathematical model for STDP can be written as follows:
\begin{equation} 
\label{eq:stdp}
\Delta w=\begin{cases} 
\Delta w^+ = A^+e^{\frac{-\Delta t}{\tau ^+}}, \text{ if } \Delta t> 0\\
\Delta w^- = A^-e^{\frac{\Delta t}{\tau ^-}}, \text{ if } \Delta t\leq 0
\end{cases}
\end{equation}
where $\Delta t=t_{post}-t_{pre}$. Essentially, this equation suggests that the synapse is potentiated (depotentiated) if post-synaptic spike happens after (before) the pre-synaptic one. $A^+$ and $A^-$ govern the maximum weight change while $\tau^+$ and $\tau^-$ dictate the time interval over which spiking activity is considered. Figure \ref{fig:stdp_theory} plots the above equation. Since this rule only deals with pairs of spikes, it is sometimes referred to as pairwise or doublet STDP. Though the above formulation uses absolute change of weight, other formulations \cite{song_stdp} use the same temporal dependence on relative weights ($\frac{\Delta w}{w}$). 

Several variants of the simple STDP rule have been proposed to better match experimental data. One of these variants is the triplet rule \cite{triplet_stdp} where the $\Delta w$ depend not only on pre-post differences but pre-pre and post-post timing differences as well. It has been shown that augmenting the simple doublet rule with these added terms allows STDP to generalize to spike trains and behave similar to BCM learning rules\cite{triplet_stdp}. FGMOS and memristors, to be introduced in the following section \ref{sec:devices}, have been used to implement STDP. Further, circuits to implement STDP in CMOS will be described in Section \ref{sec:circuits}.

\subsection{Spike Driven Synaptic Plasticity (SDSP)}
\label{sec:sdsp}
The simple doublet STDP rule does not generalize well to spike train stimulii in lerning experiments. Also, as mentioned earlier, it is unable to replicate biological measurements such as dominance of LTP at higher frequencies independent of spike timing differences. Hence, a more advanced rule has been proposed\cite{brader_sdsp,fusi_sdsp} that takes into account post-synaptic depolarization ($V(t)$) as well as post-synaptic firing rates (captured in a Calcium variable $C(t)$). The synapses in this rule are bistable with weights of $J_+$ and $J_-$ for potentiated and depotentiated states respectively. However, there is an internal analog variable $X(t)$ that governs the transition between these states as shown in the following equations:
\begin{equation} 
\label{eq:sdsp}
X=\begin{cases}
X+a \text{ if } V(t_{pre})>\theta_v \text{ and } \theta_{up}^l<C(t_{pre})<\theta_{up}^h \\
 X-b \text{ if } V(t_{pre})\leq\theta_v \text{ and } \theta_{down}^l<C(t_{pre})<\theta_{down}^h
 \end{cases}
\end{equation}
where $a$ and $b$ are jump sizes, $\theta_V$ is voltage threshold (not related to neuron's spiking threshold) and $\theta_{up}^h$, $\theta_{up}^l$, $\theta_{down}^h$ and $\theta_{down}^l$ are thresholds on the calcium variable. The synaptic weight depends on this internal variable $X$ in the following way:
\begin{equation} 
\label{eq:sdsp_weight}
w=\begin{cases}
J_+ \text{ if } X>\theta_X \\
 J_- \text{ if } X\leq\theta_X 
 \end{cases}
\end{equation}
In the absence of spikes, the variable $X$ drifts to one of two states $X_{max}$ or $X_{min}$ depending on whether $X$ is larger or smaller than $\theta_X$. The corresponding equations are:
\begin{equation} 
\label{eq:sdsp_drift}
\frac{dX}{dt}=\begin{cases}
\alpha \text{ if } X_{max}\geq X>\theta_X \\
 -\beta \text{ if } X_{min}\leq X\leq\theta_X 
 \end{cases}
\end{equation}
One major advantage of this rule is that, since the synaptic weights are binary, it can be easily implemented in CMOS hardware\cite{rolls,fusi_sdsp,mayr_swcap} without using NVM devices. Example of such hardware is presented in Section \ref{sec:bi-stable_synapse}. The dynamics of learning in such networks may be different from ones with high resolution weights especially in recurrent networks and needs to be carefully studied in future.


\subsection{Structural Plasticity}
\label{sec:struct}
While most learning algorithms in neuromorphic systems are related to the change in synaptic weights, the network structure of adult brains also undergo considerable plasticity with new connections being formed and old ones being eliminated\cite{struct_bio1,struct_bio2,struct_bio3}. In contrast to weight plasticity, this mechanism is termed as structural plasticity (SP). The advantage of considering SP in neuromorphic systems is that presence or absence of connections can be indicated by $1$-bit signals that are easy to store in CMOS latches with low write energy and cell area\cite{CICC11:SEO,mayr_swcap}. Only recently these algorithms have been applied to real world classification problems \cite{struct_frontiers,struct_shaista_neco}. To overcome the loss in computational power due to $1$-bit synapses, these \textcolor{red}{works} have used more complex neurons with multiple nonlinear dendrites. While \cite{struct_frontiers,struct_shaista_neco} applied the concept to non-spiking inputs and rate based spike trains, \cite{struct_tempo,struct_unsup} have applied SP to learn spike time based inputs. Both supervised\cite{struct_shaista_neco,struct_frontiers,struct_lsm,struct_tempo} and unsupervised versions\cite{struct_unsup,struct_liquid} of the SP algorithm have been presented. It has been also used in reservoir computing to improve the reservoir in an unsupervised fashion \cite{struct_liquid} and also to act as the readout layer\cite{struct_lsm}.

The major concept of the SP algorithm may be summarized as follows:
\begin{itemize}
\item Create network with sparse synaptic connections--locations of each synapse are therefore important.

\item Obtain $\Delta w_{ij}$ using your supervised or unsupervised weight update algorithm of choice. For example, \cite{struct_frontiers,struct_shaista_neco} uses gradient descent, \cite{struct_unsup} uses STDP while \cite{struct_tempo} uses the tempotron\cite{tempotron} as the weight update algorithm. Also, hardware friendly approximations to the actual $\Delta w_{ij}$ may be done\cite{struct_shaista_neco,struct_lsm}.

\item Instead of updating weight by adding $\Delta w_{ij}$, consider it as a fitness value $C_{ij}$. Synapses with low fitness values are candidates for replacement.  

\item Instead of random replacement, create a randomly selected candidate set for replacement. Evaluate fitness of these synapses in next iteration and choose the synapse with highest fitness value in the replacement set to replace the earlier selected synapse for replacement.

\item Repeat above steps till some pre-defined convergence criteria is met.
\end{itemize}

One of the major advantages of this learning rule is the use of $1$-bit synapses. Also, since the network has sparse synaptic connections, number of synapses used is far less compared to fully connected networks as can be seen in Table \ref{tab:algo_comparison}. Also, changes of connections can be easily implemented in address event representation (AER) based spiking systems\cite{rolls,bistable_mitra,mayr_swcap,bistable_arthur} where a separate memory stores network connection details. While the inference part of this network has been implemented\cite{struct_hw}, an area of future focus should be implementation of online learning. However, the fitness value is still stored in high resolution (4-5 bits) in current algorithms\cite{struct_unsup} and needs to be reduced for more efficient VLSI implementation of online learning systems.

\subsection{Others}
\label{sec:others}
\subsubsection{Online update for Random Neural Networks}
Recently, a class of shallow neural networks with random weights in the first layer have become popular due to their fast training speed, good generalization abilities and need for less training data. Termed extreme learning machine (ELM) \cite{elm_neurocomp} in the machine learning community, it has relations to earlier machine learning methods\cite{rvfl} as well as methods proposed in computational neuroscience\cite{nef,lsm}. Compared to the reservoir computing methods \cite{lsm}, the major difference of ELM is the lack of feedback or recurrent connections. Due to the majority of weights in the network being random, it is very amenable to neuromorphic analog implementations\cite{elm-spike-mismatch,elm_enyi,elm_chetan,elm_patil}. Since only the second layer (output layer) of weights need to be trained, it requires very few weight updates. A supervised online training algorithm for this network is proposed in \cite{opium}; however, it requires many multiplications for each output weight update. Hence, a simplified version of this algorithm called Sign based Online Update Learning (SOUL) has been developed in \cite{soul_chetan}. The learning rule is given by the following equation:
\begin{equation}
\label{eq:soul}
\overline{\Delta w_{ij}} = \alpha sgn(e_i)sgn(h_j)
\end{equation}
where $w_{ij}$ is the weight connecting j-th hidden neuron to i-th output, $sgn()$ denotes the signum function, $e_i$ is the error in the i-th output, $h_j$ denotes output of the j-th hidden neuron and $\alpha$ is a learning rate. This update can be computed using a simple XOR gate and can be used to increment weights stored in counters. It can be shown\cite{soul_chetan} that this rule is related to a version of the LMS rule.

\subsubsection{Clustering--k-means}
Clustering algorithms such as $k$-means are a class of popular unsupervised algorithms that are simple enough for low-power VLSI implementation\cite{fg_holleman}. In this method, the assumption is that the input data belongs to several classes with inter-class distance larger than intra-class distance. The objective of the learning algorithm is to learn the correct cluster centers ($\mu$) and cluster spread ($\sigma$). \cite{fg_holleman} present an FGMOS based implementation of this algorithm and achieves very high computational efficiency ($>1$Tops/W).

\subsubsection{Sparse coding--SAILnet}
With the seminal work of Olshausen and Field \cite{sparse_bruno} that showed emergence of receptive fields similar to biology when sparse representation constraints are applied, a number of works have been devoted to exploring neural architectures for finding optimal sparse codes\cite{lca} and dictionaries\cite{sailnet}. The advantage of having sparse activations from a hardware viewpoint is that few neurons will spike in the network leading to less communication and hence less energy consumption. The algorithm proposed in \cite{sailnet} is particularly attractive for hardware implementation due to local weight update rules. It has been implemented in \cite{zhengya_sparse} to obtain low energy consumption in exchange for a small loss in classification accuracy.

\subsection{Discussion}
We present a comparison of the various algorithms on machine learning tasks in Table \ref{tab:algo_comparison}. The column denoted as precision describes the precision of weights required by the algorithm. Also, some algorithms such as SDSP and structural plasticity use a low precision weight while requiring a higher precision internal variable--this is denoted by `internal' in the same column. On the other hand, algorithms like RUSD and pipelined backpropagation use a higher precision weight while the internal variable is low precision.

Another important aspect is computational complexity of the weight update. Since there is no direct correspondence between non-spike methods such as backpropagation and spike based rules such as STDP, we instead compare the computational complexity per weight update (non-spike) or per spike (spike) in Table \ref{tab:algo_comparison}.Though a direct comparison between a spike and a non-spike algorithm is difficult, it is feasible to compare the computational complexity of algorithms within spike or non-spike category.

Now, if a neural network has $M$ layers and the number of neurons in each layer is $n_i$ ($i=1,2..M$), for one backward pass the primary computations for weight update are multiplications. The number of such multiplications is given by:
\begin{equation}
\label{Backpropagation_Complexity}
C=\sum_{i=1}^{i=M-1}n_i\times n_{i+1}
\end{equation} 
Though there will be more operations required to add biases, compute gradients etc., it will not change scaling. So, the computational complexity for backpropagation will be $\mathcal{O}{(C)}$. Computational complexity of RBP and eRBP is same as regular backpropagation. For the pipelined backpropagation approaches, the computation time and hardware complexity is reduced by parallelizing the layer-wise computations and reducing the memory fetches. For RUSD, larger weight updates are applied with low probability. So, even though the theoretical complexity is same as backpropagation, actual number of computations is scaled down by a factor of $p$, the learning probability. 

The SOUL algorithm uses weight updates only in the penultimate layer. So, if the number of output nodes is $K$ and number of hidden nodes is $L$, the number of multiplications required is $K \times L$. Moreover, each multiplication here is equivalent to a bitwise XOR operation which further reduces the hardware cost of implementing it. 



Among spike based algorithms, STDP employs a local learning rule. So, if a post-synaptic spike happens in a neuron and there are $N$ pre-synaptic neurons connected to it, the $N$ synaptic weight updates are to be computed. For SDSP, though the number of weights updated per post-synaptic spike is same as STDP, additional hardware complexity is required to calculate the internal analog variable $X(t)$ as described in \cite{fusi_sdsp}.

The weight update rule is local for STDP, SDSP and eRBP while other algorithms use global weight update rules. For the SOUL algorithm, the convergence speed is fast as the weight update is applied to a single layer while for backpropagation variants the convergence is relatively slower. For the unsupervised and semi-supervised methods, it is difficult to compare the speed of convergence as it is highly dependent on the specific problem and the dataset characteristics.

==> random_novel_devices.tex <==
\section{Novel devices}
\label{sec:devices}
In this section, we review some of the novel devices that have been proposed over the years to perform the functions of neurons, synapses or adaptive elements, in general. Without losing generality, the relationship between the activity patterns of the input neurons $\textbf{\textit{x}}$ and the output neurons $\textbf{\textit{y}}$ in a NN can be expressed as:

\begin{equation} 
\label{eq:y=Wx}
\boldsymbol{y}_{n}=\boldsymbol{W}_{n \times m} \boldsymbol{x}_{m}
\end{equation}
Most of the novel devices have been used to implement the synaptic function that is denoted by $W$ in the equation \ref{eq:y=Wx}. Some desireable properties of adaptive synapses are:
\begin{itemize}
\item \textbf{Non-volatile weight} storage is required so that the effect of learning is not lost with passage of time.
\item \textbf{Compact size} is desired since the number of synapses is at least an order of magnitude larger than the number of neurons.
\item \textbf{Low energy} operation for both creation of EPSC as well as for adaptation is required. In terms of non-volatile memory units used as synapses, these correspond to `read' and `write' energies.
\end{itemize}

\subsection{Floating-Gate MOS}
\label{sec:fgmos}
\begin{figure}[!t]
\centerline
{\includegraphics[width=0.5\textwidth]{fg_combo.png}}
\caption{Circuit schematic (a) and layout (b) (taken from \cite{twigg_thesis}) of a floating-gate MOS (FGMOS). A FGMOS has all signals coupled to its gate through capacitors. The charge stored on the gate can be modified by quantum mechanical processes of electron tunneling and hot electron injection.}\label{fig:fgmos}
\end{figure}
Historically, one of the earliest non-volatile storage elements proposed as a learning synapse was the floating-gate MOS (FGMOS)\cite{stls_hasler,fg_app4}. As shown in Figure \ref{fig:fgmos}(a), a FGMOS has a regular PMOS but with no direct resistive connection to the gate. All signals are coupled capacitively to the gate of the transistor making it a floating node surrounded on all sides by high quality insulating oxide. The voltage on the floating node, $V_{fg}$ depends on the stored charge on this node along with values of other coupling voltages. This stored charge can be modified by the quantum mechanical processes of hot electron injection (HEI) and Fowler-Nordheim tunneling \cite{basu_fgprog}. Learning or adaptive systems using FGMOS modify this stored charge according to some pre-defined algorithm. 

Due to its compatibility with CMOS, FGMOS devices have been integrated into various adaptive neuromorphic circuits in the past such as competitive learning\cite{fg_app1,jen_rev_c,jen_rev_d}, offset calibration in amplifiers, comparators and voltage references\cite{fg_app3,fg_app5,jen_rev_e,jen_rev_f,jen_rev_g}, adaptive filters\cite{fg_app2,fg_app7,jen_rev_h}, removing fixed pattern noise in imagers\cite{fg_app6,jen_rev_i}, field programmable analog arrays\cite{basu_fpaa,mixed_fpaa,jen_rev_j}, synapses with spike time dependent plasticity (STDP) \cite{shubha_stdp,brink_learning_fg,roshan_doublet,roshan_triplet} and others\cite{fg_review}. Due to the ability of using a single transistor as a learning synapse in neuromorphic systems and ability to integrate tightly with CMOS circuits\cite{hasler_roadmap}, FGMOS is a good potential candidate for building large scale adaptive neuromorphic systems. A comparison of different uses of the FG device is presented in Table \ref{tab:fg_comparison}. A comparison between FG and non-FG synapses is presented in \cite{review_mostafa}.

For the recently popular case of STDP learning, we can analyze the energy per write by first noting that weight, $w$ can be expressed as:
\begin{align} 
\label{eq:fg_weight}
w=e^{\frac{\Delta V_{fg}}{U_T}}
\end{align}
where $\Delta V_{fg}$ is the slow time scale change in the FG voltage\cite{shubha_stdp,roshan_doublet} and $U_T$ denotes thermal voltage. Thus, for a maximum change in weight of $10\%$, $\Delta V_{fg}\approx 2.5$ mV at room temperature. Now, we can write the energy/write due to tunneling ($E_{tun}$) and injection ($E_{inj}$) in terms of $\Delta V_{fg}$ as follows:
\begin{align} 
\label{eq:fg_energy}
E_{tun}&=C_{tot}\Delta V_{fg}(V_{tun}-V_{fg}) \\
E_{inj}&=\frac{C_{tot}\Delta V_{fg}}{\alpha}(V_{ds,inj})
\end{align}
where $C_{tot}$ denotes total capacitance on the gate, $V_{tun}$ denotes the applied tunneling voltage, $\alpha$ denotes the injection efficiency of generation of hot-electrons\cite{fg_physics} and $V_{ds,inj}$ is the high drain-source voltage applied for injection. It should be noted that $\alpha$ is a function of $V_{ds,inj}$. While it may be argued that part of this energy is needed anyway for normal read operation (i.e. generation of EPSC), these equations still give us a method to estimate the energy/spike needed in FG synapses. As an example, by lowering $C_{tot}$ to $50$fF and keeping $V_{tun}-V_{fg}=10$V, we can estimate the $E_{tun}$ for $10\%$ weight change to be only $1.25$ fJ. $E_{inj}$ is typically much larger ($1.25-12.5$pJ) due to small values of $\alpha$ ($\approx10^{-3}-10^{-4}$)\cite{fg_physics}. 

\begin{table*}[htbp]
\centering
\caption{Comparison of fabricated floating-gate (FG) based adaptive element design for neuromorphic systems}
\label{tab:fg_comparison}
\begin{tabular}{@{}p{1cm}p{1.3cm}cp{1.5cm}cp{2cm}p{5cm}@{}}
\toprule
Ref     & Process (L in $\mu m$) & Mode      & Algorithm          & Energy & Area ($\mu m^2$) (divided by $L^2$) & Remarks                                                                     \\ \midrule
\cite{shubha_stdp} & 0.35 & Spike     & D-STDP             & -           & 100 (816)                                & Single device measured                                                      \\
\cite{brink_learning_fg} & 0.35 & Spike     & D-STDP             & 20 pJ/spike & 133 (1088)                               & 100 neurons, 10K fixed synapses, 20K plastic synapses                       \\
\cite{roshan_triplet} & 0.35 & Spike     & T-STDP             & 52 pJ/spike & 6337 (51730)                             & Single device measured, can reduce to $0.52$ pJ/spike by reducing $C_g$ to $50$ fF \\
\cite{fg_holleman}  & 0.13 & Non-spike & k-means clustering & 2 pJ/op     & -                                        & Op includes other analog operations apart from FG write                     
\\ 
\cite{hasler_lms} & 0.5 & Non-spike & LMS & - & - & 2 FGMOS based correlating synapse measured
\\
\cite{fg_app2} & 0.35 & Non-spike & LMS & 1 pJ/op & - & $48$-tap, adaptive FIR filter with digital input and analog output with 10 bits of resolution
\\
\bottomrule
\end{tabular}
\end{table*}

\subsection{Memristors}
\label{sec:memristor}

Emerging nonvolatile memory (NVM) denotes a series of new types of memory technologies that does not \textcolor{red}{rely} on electrical charge to store the data (e.g., as SRAM and DRAM). Some representative embedded NVM (eNVM) technologies are phase change memory (PCM) \cite{li2011nonvolatile}, spin-transfer-torque random-access-memory (STT-RAM) \cite{chen2010design}, resistive random-access-memory (RRAM) \cite{chen2010pcmo}, ferroelectric field-effect-transistor (FeFET) memory \cite{bayram2016adaptive} etc. Many of these eNVM technologies can be utilized to implement neuromorphic computing systems (NCS) where the programmable resistance of the eNVM cells represents the synaptic weights of the DNNs, especially RRAM (a.k.a. memristor).
The first explicit theoretical depiction of memristor was given by Leon Chua in 1971 \cite{chua1971memristor} though earlier references to a similar element may be found in Bernard Widrow's work \cite{memistor}. The resistance state (often referred to as memristance) of a memristor can be tuned by applying an electrical excitation. In 2008, HP Labs reported that memristive effect was realized by moving the doping front along a $TiO_{2}$ thin-film device \cite{strukov2008missing}, as conceptually illustrated in Figure \ref{fig:RRAM}. Here w, $\lambda$, and (D-w-$\lambda$) are the lengths of conductive region, transition region, and insulating region, respectively. $n_{s}$ is the electron density and the subscript $s=(c, t, i)$ denotes the parameter of these three regions.

\begin{figure}[!t]
\centerline
{\includegraphics[width=0.4\textwidth]{RRAM.png}}
\caption{Operating mechanism of a metal-oxide memristor. \cite{zhang2013compact}.}\label{fig:RRAM}
\end{figure}

Similarity between the programmable resistance state of memristors and the variable synaptic strengths of biological synapses dramatically simplifies the design of NCS. Figure \ref{fig:RRAM-Crossbar} shows a memristor-crossbar-based NCS. With reference to equation \ref{eq:y=Wx},$\textbf{\textit{x}}$ is mimicked by the input voltage vector (or spikes) applied on the word-line (WL) of the memristor crossbar. Every memristor is programmed to the resistance state representing the weight of its corresponding synapse. The current on each bit-line (BL) of the memristor crossbar is collected and converted to the output voltage vector y by post-processing circuitry such as comparators or integrators. The $\textbf{\textit{W}}_{n \times m}$ is often realized by two memristor crossbars, which respectively represents the positive and negative elements of the $\textbf{\textit{W}}_{n \times m}$.

\begin{figure}[!t]
\centerline
{\includegraphics[width=0.5\textwidth]{RRAM-Crossbar.png}}
\caption{Memristor-based NCS \cite{hu2014memristor}.}\label{fig:RRAM-Crossbar}
\end{figure}

\subsection{Spintronic Devices}
\label{sec:spintronic}
Recent advancement in spintronic research has shown path towards ultra-low voltage, low current and energy-efficient computing beyond traditional CMOS. These devices exploit the new materials, device designs as well as novel switching phenomena such as spin-torque-transfer (STT), domain-wall (DW) movement, spin-hall effect (SHE), spin-orbital torque (SOT), and magnetoelectric (ME) switching~\cite{locatelli2014spin,burr2017neuromorphic,chen2008design}. These innovations not only augment energy-delay scaling roadmap in CMOS systems with disruptive solutions in energy-efficient power management, dense on-die non-volatile memories, non-volatile logic, etc., but also expand the computing paradigm with non-von Neumann architectures (e.g. neuromorphic hardware). In particular, explorations in spin-based neurons and spin-based synapses to mimic biological functionality in human brains have shown potential to achieve cognitive functionality comparable with CMOS digital hardware. They may also offer much less energy consumption close to biological operations owning to the ``compact functionality'' in one single device \cite{locatelli2014spin}. These neuron-synapse systems have been benchmarked with CMOS hardware in simulation, showing significant advantages in terms of power and energy-efficiency in the range of a few to hundreds of times improvement with desired recognition accuracy \cite{sharad2012spin,sharad2013spin,sengupta2015spin,sengupta2015spin,sengupta2016magnetic,sengupta2016probabilistic,fan2016hierarchical,zhang2016all,vatajelu2017fully,jaiswal2017proposal}. In the following section, we discuss the recent progress in spin-based neurons and spin-based synapses, respectively. Note that spintronics has also been utilized to build nanoscale coupled oscillators for a different type of neuromorphic architecture \cite{torrejon2017neuromorphic}, which will not be covered in the scope of this discussion.

\textbf{Spin Neurons:}

Magnetic tunnel junctions (MTJ), well-known for on-die non-volatile memory applications, have also been investigated as the "spin neuron" candidate. A two-terminal MTJ is typically composed of two ferromagnetic layers separated by an oxide tunnel barrier. One layer has fixed spin polarization, namely pinned layer (PL), and the other free layer (FL) can alter its polarization depending on the spin current through the MTJ via spin-transfer-torque (STT) effect. Depending on its parallel (P) or antiparallel state (AP) with respect to the PL, the resistance of the MTJ can be low resistance for P or high resistance for AP. Since the MTJ switching is governed by a critical current, the analogy to the thresholding effect in biological neuron (that accepts the weighted input from synapse) has been explored to build the biological neuron model. 
\begin{table*}[!htbp]
\footnotesize
\centering
\caption{Summary of Spin neuron and synapse devices (Simulation)}
\label{tab:spin_comparison}
\begin{adjustbox}{width=\linewidth}
\setlength\tabcolsep{1.5pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{ | m{0.17\linewidth} | m{0.28\linewidth} | m{0.14\linewidth} | m{0.14\linewidth} | m{0.12\linewidth} | m{0.17\linewidth} |}
\hline
\rowcolor[HTML]{5B9BD5} 
{\color[HTML]{FFFFFF} \textbf{Device Type}}  & {\color[HTML]{FFFFFF} \textbf{Circuit Topology}} & {\color[HTML]{FFFFFF} \textbf{Energy}}  & {\color[HTML]{FFFFFF} \textbf{Accuracy}} & {\color[HTML]{FFFFFF} \textbf{Applications}}&{\color[HTML]{FFFFFF} \textbf{Cost}} \\ \hline
\rowcolor[HTML]{DEEAF6} 
MTJ neuron and DWM synapse system \cite{sharad2012spin,narasimman2016low} & \includegraphics[width=\linewidth]{img/MTJ_DWM.png} & Average 51fJ/neuron \cite{sharad2012spin}; 40fJ/weight update with online learning \cite{narasimman2016low} & 95.4\% for handwriting digit recognition \cite{narasimman2016low} & ANN implementation for pattern detection in MNIST & 1 DWM per synapse, 1 MTJ per neuron, preset magnet and CMOS sensing/signaling circuits (8T with ref. MTJ). Additional STDP function write circuits (10T). \\
DWM neuron \cite{sharad2013spin,fan2016hierarchical} & \includegraphics[width=\linewidth]{img/DWM.png} & 48pJ for a single HTM level-2 node design \cite{fan2016hierarchical} & Max 95\% of matching threshold of 0.7 \cite{fan2016hierarchical} & HTM inference hardware mapping with offline training &1 3-terminal DWM device per neuron, CMOS sensing circuits (1 INV or 7T latch with ref. MTJ). CMOS DAC and 5-bit SAR ADC.\\
\rowcolor[HTML]{DEEAF6} 
MTJ neuron with SOT assist \cite{sengupta2016magnetic,sengupta2016probabilistic} & \includegraphics[width=\linewidth]{img/MTJ_SOT.png}  & 19.5nJ per image operation \cite{sengupta2016probabilistic} & 83\% for 0.2ns write time; 97\% for 1ns write time \cite{sengupta2016probabilistic} & Stochastic neuron; MNIST image recognition &1 3-terminal MTJ HM device per neuron, CMOS readout circuit (1 INV with ref. MTJ).\\ 
DWM synapse with SOT \cite{sengupta2015spin} & \includegraphics[width=\linewidth]{img/DWM_SOT.png} & $\sim$2pJ per synaptic event \cite{sengupta2015spin} & N/A & STDP implementation &1 3-terminal MTJ DWM HM device with 4 CMOS access transistor per synapse and CMOS signaling post-neuron summing amplifier.\\
\rowcolor[HTML]{DEEAF6} 
ME neuron \cite{jaiswal2017proposal} & \includegraphics[width=\linewidth]{img/ME.png} & 246fJ per neuron per training iteration & 80\% with 1600 ME neurons  & Stochastic LIF neuron implementation &1 ME with MTJ per neuron, CMOS signaling/sensing circuits (4T1R and ref MTJ).\\
Multi-level MTJ neuron and synapse \cite{zhang2016all} & \includegraphics[width=\linewidth]{img/Multi-level_MTJ.png} & N/A & 91\% with 60k training; 84\% with 30\% variation with 3 MTJ & Digital pattern recognition in MNIST&1 multi-level MTJ per neuron with CMOS signaling/sensing circuits (5T control circuits and 1 amplifier) \\
\rowcolor[HTML]{DEEAF6} 
MTJ array synapse \cite{vatajelu2017fully} & \includegraphics[width=\linewidth]{img/MTJ.png} & N/A & 93\% - 88\% with 16 MTJ for min to max device-to-device variation & Digital pattern recognition in MNIST & Multiple MTJ per synapse (1~16), 1 MTJ per neuron with CMOS sensing/ signaling circuits (7T control circuits, 1 amplifier, 1 pulse generator) \\ \hline
\end{tabular}}
\end{adjustbox}
\end{table*}
Sharad et al. \cite{sharad2012spin} proposed using a lateral spin valve (LSV), where an MTJ is connected to multiple domain wall magnet (DWM) based synapses (will be discussed later) and receives spin-weighted input current from a non-magnetic, metal channel. The metal channel sums the spin-polarized charge current and contacts the free layer of the MTJ. This current switches MTJ through nonlocal STT switching if it is above the critical value. The change of the MTJ resistance is then detected by a differential MTJ latch to generate a ``spike" to the gate of a PMOS transistor that connects to the receiving synapse. Recently, Narasimman et al. \cite{narasimman2016low} developed circuit solution to implement spike-timing-dependent-plasticity (STDP) based on this DWM-synapse and MTJ-neuron system by sampling pre- and post-synaptic time, showing on-line learning capability with significant energy-efficiency improvement.

Sharad et al. also proposed another approach \cite{sharad2013spin,fan2016hierarchical} using a three-terminal DWM with SHE assist and MTJ, where a free domain in DWM strip forms an MTJ with a tunnel barrier and a fixed magnet on top. Two fixed domains in opposite polarization states are separated by the free domain. During inference, the weighted and summed charge current from synapse crossbar connects to one terminal of the DWM (one of the fixed domain), which can move the DW depending on the current direction and thereby changes the MTJ resistance. This is sensed by a reference MTJ and connected to a CMOS inverter to generate a ``spike''. The SHE layer underneath the DWM strip improves the DW velocity. 

Besides LSV and DWM, Sengupta et al. \cite{sengupta2015spin} further proposed a SOT-based neuron using ferromagnet/heavy metal (FM/HM) device, where the free layer of the MTJ contacts the HM. The thresholding is achieved with 2-step control, where a clock current through HM to first orient MTJ FL to unstable point, then the write current through MTJ performs deterministic switching. The SOT effect by the clock current helps to minimize the required current and further improve the energy-efficiency.

With recent theoretical studies on probabilistic spiking nature of pyramidal neurons, Sengupta et al. \cite{sengupta2016magnetic,sengupta2016probabilistic} employed the stochastic switching of MTJ as a function of current to mimic such neuron behavior. The write current (sum of the weighted input) through the HM to switch the MTJ follows a similar sigmoid probability density function, which (1) takes into account spintronic device variation nature and (2) allows mapping of graded analog transfer function in artificial neural network (ANN) to spiking neural network (SNN). 

Given the binary switching nature of MTJ, the above approaches still fail to model the analog behavior of membrane potential. While leaky-integrate-fire (LIF) model has shown its capability to closely model neuron dynamics and been adopted in CMOS neuromorphic hardware, Jaiswal et al. proposed the LIF implementation using magnetoelectric (ME)-oxide-ferromagnet heterostructure to model stochastic-LIF neuron \cite{jaiswal2017proposal}. Two transistors are added for synaptic input and leaky/reset, respectively, and the ME switching alters ferromagnet state. An MTJ formed by ferromagnet-MgO-pinned layer is used for reading and generating the spike with a reference MTJ and inverter. Given ME switching is charge-dependent and stochastic, the leaky-integrate-fire operation can be realized.

Another approach to achieve the analog neuron is to use multi-level MTJ \cite{zhang2016all}. Zhang et al. used a vertical stacked MTJ for both neuron and synapse to enable multi-step transfer function. Additional three NMOS transistors are used to perform reset, read and accepting synapse input, and one CMOS amplifier is used and MTJ is connected as feedback resistor (no need for reference MTJ). The higher the multi-level MTJ resistance, the higher the output voltage. Vatajelu et al. \cite{vatajelu2017fully} further employed the similar configuration with MTJ but connecting the output spike voltage to synapse input for STDP modulation on synapse.

In all the described spin-neuron implementation, a “reset" is always required after firing in order to restore the nanomagnet to its reference state. 

\textbf{Spin Synapses:}

Besides the memristor-crossbar-based synapse, spintronic devices can also be used to implement synaptic operation. In \cite{zhang2016all}, Zhang et al. used the vertical stacked multi-level MTJ for synapse which can achieve 4 different levels. Since increasing the number of level imposes changes on device fabrication, \cite{vatajelu2017fully} Vatajelu et al. further proposed $2^{nd}$ level crossbar connection for a single synapse (e.g. 3$\times$3 connection with 9 MJT for a 10-level synapse), and showed the reduction in recognition error rate with improvement of synapse levels. DWM, owning to its displacement and spin-polarization current dependency, has also been used for synapse implementation. In all-spin based neuron-synapse system, Sharad et al. \cite{sharad2012spin} used DWM to connect to spin neuron through metal channel, where the DW location is programmed off-line. The location of DW during inference modulates the spin-polarization current for spin neuron switching. However, DWM synapses may be limited by fanout number, spin diffusion length, number of levels (require long DWM strip), which are in research phase. Narasimman et al. \cite{narasimman2016low} further implement STDP for DWM synapse to enable on-line learning. In \cite{sengupta2015spin}, Sengupta et al. proposed a four-terminal ferromagnet-heavy metal heterostructure to implement STDP, which combines the MTJ with the DWM as free layer which contacts an HM. The learning is done through SOT by using the charge current through HM and applied magnetic field to modulate the DW displacement, while the reading is through MTJ and non-magnetic contact on the HM (decoupled current path for learning and reading). The transistors are connected to pre-spike and post-spike signals which modulate the DW based on the neuron firing activity. Comparing to memristor synapse approach, DWM synapse shows lower current operation due to the SHE enhanced spin injection efficiency which helps to reduce the power consumption per synaptic operation.

A summary of both spin neurons and synapses reported so far is presented in Table \ref{tab:spin_comparison}.Comparing with CMOS-based approaches, spintronic devices offer opportunities to realize compact neuron and synapse models with a potential energy-efficiency improvement (e.g. lower supply voltage ($<$1V) and lower current compared to memristor and floating gate \cite{narasimman2016low,spin_kroy_tcas1,spin_sot_STDP}). The low current requirements have a direct effect on noise and hence special stochastic algorithms might be needed to train these networks\cite{spin_review_kroy}. Nevertheless, most of these devices still require CMOS circuits for signal propagation, control, sensing or functionality. Since most of the works are still in early research phase and simulation stage, main challenges remain in large-scale device demonstration including variation and reliability, novel material integration, spin injection efficiency improvement, etc and all improvements in simulation should be considered as potential gains only.



\subsection{Discussion}
Among the floating-gate circuits reported in Table \ref{tab:fg_comparison}, the earliest ones were non-spiking ones where \cite{fg_app2} used the same LMS algorithm as \cite{hasler_lms} but reduced technology node. Recent work \cite{fg_holleman} has used k-means as well as reduced technology node further to $0.13\mu$m  CMOS. Among the STDP implementations, \cite{shubha_stdp} was the first implementation of STDP on a FG device while \cite{brink_learning_fg} actually implemented an array with neurons and AER. \cite{roshan_triplet} implemented a more advanced version of the STDP rule including triplet spike interactions.

An important consideration for all adaptive elements to be used in neural network algorithms is intrinsic mismatch in programming desired weight values. Very few work have tried to explicitly correct the mismatch in a structured way, with \cite{biocas_mismatch_sun} being one exception. In some specific cases, mismatch may be used in the computation \cite{elm_enyi} but these methods may require $2-3X$ more neurons. Moreover, they have not yet been shown for a general multi-layered network. FG based adaptive elements have been used for nearly three decades and have a much better control on statistical variations than their memristive counterparts. The usage of HEI as programming mechanism is also motivated by this fact since mismatch is much less than tunneling junctions\cite{jen_rev_a}. Memristors typically show $2-3$ bits of accuracy in large arrays\cite{memristor_sparse} and only recently, there have been reports of $\approx 6$ bits of accuracy\cite{memristor_vmm}. In Table \ref{tab:algo_comparison}, we show the precision requirement reported for some of the algorithms. An in-depth analysis of device mismatch in the context of these algorithms is an important direction for future work.

One attractive property for memristors over FGMOS devices is their potentially lower write energy. However, it is interesting to note that memristors suffer from poor selectivity issues in large arrays as a tradeoff. Typically, diodes are used to prevent sneak paths which lead to larger cell sizes. While the almost perfect selection of FGMOS using HEI makes system design simpler, we also see this as an opportunity to make better algorithms that are less affected by crosstalk and sneak paths in exchange for lower write energy.

Spin devices are a much more recent development with fewer published work and hence we have also reported neurons implemented in spintronic technology. For discussions on CMOS neurons, readers are referred to \cite{neuron_review} and references therein.

==> temp.tex <==
\noindent
====================

\noindent
\textbf{[This section is Tanay's part on spintronic technology.]}

AUTHORS of this Section: Huichu Liu, Tanay Karnik, Microarchitecture Research Lab, Intel Labs

II. Novel Devices:

\textbf{Spintronic Devices for Neuromorphic Computing:}

Recent advancement in spintronic research has shown path towards ultra-low voltage, low current and energy-efficient computing beyond traditional CMOS. Those devices exploit the new materials, device designs as well as novel switching phenomena such as spin-torque-transfer (STT), domain-wall (DW) movement, spin-hall effect (SHE), spin-orbital torque (SOT), magnetoelectric (ME) switching, etc \cite{locatelli2014spin,burr2017neuromorphic,chen2008design}. These innovations not only augment energy-delay scaling roadmap in CMOS systems with disruptive solutions in energy efficient power management, dense on-die non-volatile memories, non-volatile logic, etc, but also expand the computing paradigm with non-Von Neumann architectures (e.g. neuromorphic hardware). In particular, explorations in spin-based neurons and spin-based synapses to mimic biological functionality in human brains have shown potential to achieve cognitive functionality comparable with CMOS digital hardware. They may also offer much less energy consumption close to biological operations owning to the "compact functionality" in one single device \cite{locatelli2014spin}. These neuron-synapse systems have been benchmarked with CMOS hardware in simulation, showing significant advantages in terms of power and energy efficiency in the range of a few to hundreds of times improvement with desired recognition accuracy \cite{sharad2012spin,sharad2013spin,sengupta2015spin,sengupta2015spin,sengupta2016magnetic,sengupta2016probabilistic,fan2016hierarchical,zhang2016all,vatajelu2017fully,jaiswal2017proposal}. In the following section, we discuss the recent progress in spin-based neurons and spin-based synapses, respectively. Note that spintronics has also been utilized to build nanoscale coupled oscillators for a different type of neuromorphic architecture \cite{torrejon2017neuromorphic}, which will not be covered in the scope of this discussion.

\textbf{Spin Neurons:}

Magnetic tunnel junctions (MTJ), well-known for on-die non-volatile memory applications, have also been investigated as the "spin neuron" candidate. A two-terminal MTJ is typically composed of two ferromagnetic layers separated by an oxide tunnel barrier. One layer has fixed spin polarization, namely pinned layer (PL), and the other free layer (FL) can alter its polarization depending on the spin current through the MTJ via spin-transfer-torque (STT) effect. Depending on its parallel (P) or antiparallel state (AP) with respect to the PL, the resistance of the MTJ can be low resistance for P or high resistance for AP. Since the MTJ switching is governed by a critical current, the analogy to the thresholding effect in biological neuron (that accepts the weighted input from synapse) has been explored to build the biological neuron model. 

Sharad et al \cite{sharad2012spin} proposed using a lateral spin valve (LSV), where an MTJ is connected to multiple domain wall magnet (DWM) based synapses (will be discussed later) and receives spin-weighted input current from a non-magnetic, metal channel. The metal channel sums the spin-polarized charge current and contacts the free layer of the MTJ. This current switches MTJ through nonlocal STT switching if it is above the critical value. The change of the MTJ resistance is then detected by a differential MTJ latch to generate a "spike" to the gate of a PMOS transistor that connects to the receiving synapse. Recently, Narasimman et al \cite{narasimman2016low} developed circuit solution to implement spike-timing-dependent-plasticity (STDP) based on this DWM-synapse and MTJ-neuron system by sampling pre- and post-synaptic time, showing on-line learning capability with significant energy efficiency improvement.

Sharad et al also proposed another approach \cite{sharad2013spin,fan2016hierarchical} using a three-terminal DWM with SHE assist and MTJ, where a free domain in DWM strip forms an MTJ with a tunnel barrier and a fixed magnet on top. Two fixed domain in opposite polarization states are separated by the free domain. During inference, the weighted and summed charge current from synapse crossbar connects to one terminal of the DWM (one of the fixed domain), which can move the DW depending on the current direction and thereby changes the MTJ resistance. This is sensed by a reference MTJ and connected to a CMOS inverter to generate a "spike". The SHE layer underneath the DWM strip improves the DW velocity. 

Besides LSV and DWM, Sengupta et al \cite{sengupta2015spin} further proposed a SOT-based neuron using ferromagnet/heavy metal (FM/HM) device, where the free layer of the MTJ contacts the HM. The thresholding is achieved with 2-step control, where a clock current through HM to first orient MTJ FL to unstable point, then the write current through MTJ performs deterministic switching. The SOT effect by the clock current helps to minimize the required current and further improve the energy efficiency.

With recent theoretical studies on probabilistic spiking nature of pyramidal neurons, Sengupta et al \cite{sengupta2016magnetic,sengupta2016probabilistic} employed the stochastic switching of MTJ as a function of current to mimic such neuron behavior. The write current (sum of the weighted input) through the HM to switch the MTJ follows a similar sigmoid probability density function, which (1) takes into account spintronic device variation nature and (2) allows mapping of graded analog transfer function in artificial neural network (ANN) to spiking neural network (SNN). 

Given the binary switching nature of MTJ, the above approaches still fail to model the analog behavior of membrane potential. While leaky-integrate-fire (LIF) model has shown its capability to closely model neuron dynamics and been adopted in CMOS neuromorphic hardware, Jaiswal et al proposed the LIF implementation using magnetoelectric (ME)-oxide-ferromagnet heterostructure to model stochastic-LIF neuron \cite{jaiswal2017proposal}. Two transistors are added for synaptic input and leaky/reset, respectively, and the ME switching alters ferromagnet state. An MTJ formed by ferromagnet-MgO-pinned layer is used for reading and generating the spike with a reference MTJ and inverter. Given ME switching is charge-dependent and stochastic, the leaky-integrate-fire operation can be realized.

Another approach to achieve the analog neuron is to use multi-level MTJ \cite{zhang2016all}. Zhang et al used a vertical stacked MTJ for both neuron and synapse to enable multi-step transfer function. Additional three NMOS transistors are used to perform reset, read and accepting synapse input, and one CMOS amplifier is used and MTJ is connected as feedback resistor (no need for reference MTJ). The higher the multi-level MTJ resistance, the higher the output voltage. Vatajelu et al \cite{vatajelu2017fully} further employed the similar configuration with MTJ but connecting the output spike voltage to synapse input for STDP modulation on synapse.

In all the described spin-neuron implementation, a “reset" is always required after firing in order to restore the nanomagnet to its reference state. 

\textbf{Spin Synapses:}

Besides the resistive RAM (RRAM) crossbar based synapse, spintronic devices can also be used to implement synaptic operation. In \cite{zhang2016all}, Zhang et al used the vertical stacked multi-level MTJ for synapse which can achieve 4 different levels. Since increasing the number of level imposes changes on device fabrication, \cite{vatajelu2017fully} Vatajelu et al further proposed $2^{nd}$ level crossbar connection for a single synapse (e.g. 3$\times$3 connection with 9 MJT for a 10-level synapse), and showed the reduction in recognition error rate with improvement of synapse levels. DWM, owning to its displacement and spin-polarization current dependency, has also been used for synapse implementation. In all-spin based neuron-synapse system, Sharad et al \cite{sharad2012spin} used DWM to connect to spin neuron through metal channel, where the DW location is programmed off-line. The location of DW during inference modulates the spin-polarization current for spin neuron switching. However, DWM synapses may be limited by fanout number, spin diffusion length, number of levels (require long DWM strip), which are in research phase. Narasimman et al \cite{narasimman2016low} further implement STDP for DWM synapse to enable on-line learning. In \cite{sengupta2015spin}, Sengupta et al proposed a four-terminal ferromagnet-heavy metal heterostructure to implement STDP, which combines the MTJ with the DWM as free layer which contacts an HM. The learning is done through SOT by using the charge current through HM and applied magnetic field to modulate the DW displacement, while the reading is through MTJ and non-magnetic contact on the HM (decoupled current path for learning and reading). The transistors are connected to pre-spike and post-spike signals which modulate the DW based on the neuron firing activity. Comparing to RRAM synapse approach, DWM synapse shows lower current operation due to the SHE enhanced spin injection efficiency which helps to reduce the power consumption per synaptic operation.

Comparing with CMOS-based approaches, spintronic devices offer opportunities to realize compact neuron and synapse models with a potential energy efficiency improvement (e.g. lower supply voltage ($<$1V) and lower current compared to RRAM and floating gate \cite{narasimman2016low}). The non-volatility aspects of these devices can also enable aggressive power gating for leakage power reduction. Nevertheless, most of these devices still require CMOS circuits for signal propagation, control, sensing or functionality. Since most of the work are still in early research phase and simulation stage, main challenges remain in large-scale device demonstration including variation and reliability, novel material integration, spin injection efficiency improvement, etc.

\textbf{III. Circuit Innovations:}

\textbf{Spin-based interface circuits:}

Spin-based interface circuits have also been proposed to assist the operation of spin neurons and synapses. For example, to evaluate the MTJ based neuron state (firing or not), a reference MTJ in antiparallel state was connected in series with the MTJ neuron and input to an inverter. When the MTJ neuron is in antiparallel state, the inverter output is low; while MTJ neuron is switched to parallel state, the inverter output is high \cite{sharad2013spin,sengupta2015spin,sengupta2015spin,sengupta2016magnetic,sengupta2016probabilistic,fan2016hierarchical,zhang2016all,vatajelu2017fully,jaiswal2017proposal}. For all-spin based neuron-synapse system, a differential latch with MTJ was used to latch the output and drive the next spin synapse \cite{sharad2013spin}. Depending on the spintronic device operation, CMOS circuits are usually required to provide clocking and control of the signal propagation in the neural nets.

\begin{table*}[t]
\footnotesize
\centering
\caption{Spin Neuron and Synapse Devices}
\label{Comparison}
\begin{adjustbox}{width=\linewidth}
\setlength\tabcolsep{1.5pt}
\resizebox{\textwidth}{!}{
\begin{tabular}{ | m{0.17\linewidth} | m{0.28\linewidth} | m{0.19\linewidth} | m{0.19\linewidth} | m{0.17\linewidth} | }
\hline
\rowcolor[HTML]{5B9BD5} 
{\color[HTML]{FFFFFF} \textbf{Device Type}}  & {\color[HTML]{FFFFFF} \textbf{Circuit Topology}} & {\color[HTML]{FFFFFF} \textbf{Energy}}  & {\color[HTML]{FFFFFF} \textbf{Accuracy}} & {\color[HTML]{FFFFFF} \textbf{Applications}}  \\ \hline
\rowcolor[HTML]{DEEAF6} 
MTJ neuron and DWM synapse system \cite{sharad2012spin,narasimman2016low} & \includegraphics[width=\linewidth]{img/MTJ_DWM.png} & Average 51fJ/neuron \cite{sharad2012spin}; 40fJ/weight update with online learning \cite{narasimman2016low} & 95.4\% for handwriting digit recognition \cite{narasimman2016low} & ANN implementation for pattern detection in MNIST \cite{sharad2012spin,narasimman2016low} \\
DWM neuron \cite{sharad2013spin,fan2016hierarchical} & \includegraphics[width=\linewidth]{img/DWM.png} & 48pJ for a single HTM level-2 node design \cite{fan2016hierarchical} & Max 95\% of matching threshold of 0.7 \cite{fan2016hierarchical} & HTM inference hardware mapping with offline training \\
\rowcolor[HTML]{DEEAF6} 
MTJ neuron with SOT assist \cite{sengupta2016magnetic,sengupta2016probabilistic} & \includegraphics[width=\linewidth]{img/MTJ_SOT.png}  & 19.5nJ per image operation \cite{sengupta2016probabilistic} & 83\% for 0.2ns write time; 97\% for 1ns write time \cite{sengupta2016probabilistic} & Stochastic neuron; MNIST image recognition \\ 
DWM synapse with SOT \cite{sengupta2015spin} & \includegraphics[width=\linewidth]{img/DWM_SOT.png} & $\sim$2pJ per synaptic event \cite{sengupta2015spin} & N/A & STDP implementation \\
\rowcolor[HTML]{DEEAF6} 
ME neuron \cite{jaiswal2017proposal} & \includegraphics[width=\linewidth]{img/ME.png} & 246fJ per neuron per training iteration & 80\% with 1600 ME neurons  & Stochastic LIF neuron implementation \\
Multi-level MTJ neuron and synapse \cite{zhang2016all} & \includegraphics[width=\linewidth]{img/Multi-level_MTJ.png} & N/A & 91\% with 60k training; 84\% with 30\% variation with 3 MTJ & Digital pattern recognition in MNIST \\
\rowcolor[HTML]{DEEAF6} 
MTJ array synapse \cite{vatajelu2017fully} & \includegraphics[width=\linewidth]{img/MTJ.png} & N/A & 93\% - 88\% with 16 MTJ for min to max device-to-device variation & Digital pattern recognition in MNIST \\ \hline
\end{tabular}}
\end{adjustbox}
\end{table*}
